Decoupled Residual Denoising Diffusion Models for Unified and Data Efficient Image-to-Image Translation

We propose Decoupled Residual Denoising Diffusion models (DRDD) for unified and data-efficient image-to-image (I2I) translation. While diffusion models have advanced I2I translation in terms of quality and diversity, we uncover a previously under-explored property in diffusion models. Crucially, beyond its conventional role of manifold lifting (i.e., moving data off low-dimensional manifolds), injecting Gaussian noise facilitates domain harmonization by implicitly aligning feature distributions across domains, a property particularly advantageous for unified I2I translation. However, existing diffusion models prematurely erode this harmonization effect, as noise and residuals are simultaneously removed in a single coupled diffusion process. To address this, DRDD decouples the diffusion process into two sequential and independent diffusion stages: (1) a stochastic noise diffusion for domain harmonization and manifold lifting, and (2) a deterministic residual diffusion that learns the core semantic mapping entirely within the fixed-noise domain. This decoupling preserves harmonization and manifold lifting effects throughout the transformation, substantially simplifying the learning of unified mappings across diverse tasks and domains. Notably, the noise diffusion stage is trained exclusively on abundant, unpaired target-domain images, greatly improving data efficiency. Comprehensive theoretical and empirical analysis demonstrates that DRDD is broadly compatible with mainstream diffusion models and consistently delivers robust, unified I2I translation, even under limited paired data. Our code is available at https://github.com/HKU-HealthAI/DRDD.

==> pic/data_prune_1.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.99\linewidth}
        \centering
        \includegraphics[width=\linewidth]{pic/data_prune1.pdf}
        \label{fig:main_result_a}
    \end{subfigure}
    \vspace{-1em}
    \begin{subfigure}[t]{0.99\linewidth}
        \centering
        \includegraphics[width=\linewidth]{pic/data_prune2.pdf}
        \label{fig:main_result_b}
        \vspace{-1em}
    \end{subfigure}
    \begin{subfigure}[t]{0.80\linewidth}
        \centering
        \includegraphics[width=\linewidth]{pic/legend_only.pdf}
        \label{fig:main_result_b}
    \end{subfigure}
    \vspace{-2em}
    \caption{\textit{Data Pruning on All-in-One-3 \citep{instructIR} and Low-Light dataset.} SSIM ($\uparrow$) and LPIPS ($\downarrow$) are reported. As the training data decreases, DRDD's performance drop is much smaller than other methods.}
    \vspace{-1em}
    \label{fig:data_efficiency}
\end{figure}


==> pic/light.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.99\linewidth]{pic/low_light_sample.png}  % 替换为您的图片路径
    \label{fig:main_result}  % 建议添加标签便于引用
\end{figure*}

==> pic/psnr_ratio_scale.tex <==
\begin{figure}[ht]
\centering
\includegraphics[width=0.99\linewidth]{pic/psnr_ratio_scale.png}
\caption{PSNR noise scale}
\label{fig:single}
\end{figure}

==> sec/0_abstract.tex <==
% \begin{abstract}
% Universal image restoration is a practical yet challenging computer vision task, as real-world scenarios often exhibit multiple degradation patterns (e.g., noise, blur, haze, and raindrops). Existing approaches typically rely on multiple task-specific models or explicit multi-partite mappings, which overlook the shared information across different degradation distributions. In this work, we propose a novel decoupled diffusion-based restoration framework that splits the “remove-degradation” objective into two complementary sub-tasks: removing image residual and denoising. Specifically, by injecting Gaussian noise into degraded images, our framework reduces the complexity of residual correction and enables easy sharing of residual-removal knowledge across tasks, while treating the denoising process as a universal sub-module independent of specific degradation types. This selective decoupling strategy elegantly aligns different task distributions into a shared space and then guides them back into high-quality, task-specific outputs. We further introduce three distinct variants of this decoupled framework and systematically investigate their suitability across different task scenarios. Extensive experiments show that our model maintains a competitive edge over other approaches at a similar parameter scale. Beyond its state-of-the-art performance on five benchmark tasks in the universal setting, extensive experiments further demonstrate that our proposed method can maintain competitive performance even when trained using only half (or less) of the original training data, highlighting its remarkable data efficiency and flexibility for real-world image restoration.
% \end{abstract}



% \begin{abstract}
% Universal image restoration is a practical yet challenging computer vision task, as real-world scenarios often exhibit multiple degradation patterns (e.g., noise, blur, haze, and raindrops). Existing approaches typically rely on multiple task-specific models or explicit multi-partite mappings, which overlook the shared information across different degradation distributions. 

% In this work, we propose a novel decoupled diffusion-based restoration framework that splits the “remove-degradation” objective into two complementary sub-tasks: removing image residual and denoising. Specifically, by injecting Gaussian noise into degraded images, our framework reduces the complexity of residual correction and enables easy sharing of residual-removal knowledge across tasks, while treating the denoising process as a universal sub-module independent of specific degradation types. This selective decoupling strategy elegantly aligns different task distributions into a shared space and then guides them back into high-quality, task-specific outputs. 

% We further introduce three distinct variants of this decoupled framework and systematically investigate their suitability across different task scenarios. Extensive experiments show that our model maintains a competitive edge over other approaches at a similar parameter scale and inference time. Beyond its state-of-the-art performance on five benchmark tasks in the universal setting, extensive experiments further demonstrate that our proposed method can maintain competitive performance even when trained using only half (or less) of the original training data, highlighting its remarkable data efficiency and flexibility for real-world image restoration.
% \end{abstract}




% \begin{abstract}
% We propose a novel Decoupled residual denoising Diffusion framework for unified and data efficient Image-to-Image Transformation (DDIT). Different from prior diffusion-based works that directly model the generation process from noise-carrying degraded images to clear images, we decouple the domain transformation (i.e. residual-removal) and denoising into two consecutive and independent tasks, where we first remove the residual in a fixed noise space, and then perform denoising. This decoupled design offers two pivotal advantages: (i) A fixed noise space serves as a unified space that minimizes the distance between the source and target domains, and reduces the gap between different transformation tasks, leading to impressive performance in All-in-One tasks. (ii) Data Efficiency: Our method use two independent samplers in reverse diffusion process, where denoising sampler can be trained without the need of paired images, thereby alleviating the burden of collecting high quality paired training data. DDIT is compatible with multiple diffusion paradigms, including DDPM, DDIM, and SDE-based methods, and it is also adaptable to various image-to-image transformation tasks such as image restoration, image inpainting, super resolution, and image translation. Extensive experiments show that our approach outperforms state-of-the-art methods on All-in-One benchmark tasks with simple UNet architecture while maintaining comparable parameters and inference time. We also illustrate the optimal level of noise injection through empirical experiment and theoretical analysis.



\begin{abstract}
We propose a novel Decoupled residual denoising Diffusion framework for unified and data efficient Image-to-Image Transformation (DDIT). Different from prior diffusion-based I2I works that directly model the image transformation process from noisy-carrying images to clear images, DDIT decouples this process into two consecutive and independent sub-tasks, where we first conduct residual-removal (i.e., domain transformation) in a fixed noise space, and then perform general denoising. This decoupled approach allows the model to learn deterministic semantic transformation in the first stage, enabling effective cross-task knowledge sharing in a noisy space. While in the second stage, a separate model focus on denoising process, in which we don't need paired training images, leading to data efficiency. As a result, our method achieves All-in-One image transformation without the need for explicit degradation type specification. Extensive experiments show that our approach outperforms state-of-the-art methods on popular All-in-One benchmarks while maintaining comparable parameters and inference time. We also show that DDIT significantly enhances data efficiency by supporting training on small amount of paired data.


% Our framework can be divided into two steps: In the first stage, Gaussian noise is injected into the input image, mapping different degradation tasks (e.g., deraining, dehazing, and deblurring) into a shared noisy representation space, where the residual removal is then performed within this space. In the second stage, a general denoising process is performed, transforming the distributions back to high quality domain. This decoupled approach allows the model to learn deterministic semantic transformation in the first stage, enabling effective cross-task knowledge sharing. While in the second stage, the model focus on random denoising and clear image generation. 








% Additionally, the decoupling of residual removal and denoising allows the second stage's denoising process to use knowledge pre-trained on large scale natural images, improving restoration performance and generalization with limited data. Notably, with only 25\% of the training data, our method achieves a minimal 0.25dB drop, highlighting its remarkable data efficiency and practicality in real-world scenarios.


% 这段介绍
% Our framework can be divided into two steps: In the first stage, Gaussian noise is injected into the degraded image, mapping different degradation tasks (e.g., deraining, dehazing, and deblurring) into a shared noisy representation space, where the residual removal is then performed within this space. In the second stage, a general denoising process is performed. This decoupled approach allows the model to learn general semantic transformation in the first stage, enabling effective cross-task knowledge sharing. While in the second stage, the model can focus on random denoising and clear image generation. 
\end{abstract}




%写作手法一：对着钉子造锤子
%研究问题与背景定义
%研究动机与核心思想
%方法简述
%实验结果 (Experimental Results)
%资源可用性 (Optional: Availability)




%写作手法二：拿着锤子找钉子






%还缺的东西
%图片对比
%公式证明
%



%可能会被问的问题
%参数量 对比实验效果没那么好？

==> sec/1_intro.tex <==
%-----------------------------------------------------------%
\section{Introduction}



%从信噪比的角度来切入

%一句话介绍研究领域
% Move 1. 建立研究领域（Establish a research territory）
% a. 说明该总体研究领域在某种意义上是重要的、核心的、有趣的，并且存在问题。

% 扩散模型及其基于分数的变体通过向数据注入多尺度噪声并学习逆转这一过程，在图像合成方面取得了出色的效果，并已广泛用于有条件的图像生成，包括图像修复、图像补全和图像到图像翻译。

% 早期的image-conditioned generation方法通常从纯噪声图像出发，通过使用input image作为条件，隐式地指导图像生成。为了解决纯噪声中恢复不稳定的问题，一些作者尝试在生成时对齐低质量图片的信息或者从带有噪声的input image中进行图像生成。
% 在扩散模型的图像到图像转换中，早期的方法常从纯噪声出发，并通过特征拼接等显式条件注入将输入图像的信息融入去噪过程。 为在图像到图像任务中更稳定地保留输入结构并降低推理阶段的不确定性，许多方法不再从纯噪声起步，而是将输入图像先加噪到某一中间噪声水平，再运行条件扩散的反向过程，使模型在去噪的同时完成分布/域的迁移。
%在解决universal问题上 解耦的做法和SDT思路是一致的 SDT通过在前向过程中逐步减少退化图像的量来实现share，可以理解成随着噪声增多，控制input不要太多

%这个和我们的第一阶段是耦合的
%到底为什么在噪声环境里 做退化会更好  【噪声环境里 退化图像和干净图像的分布距离更小，

Image-to-image (I2I) transformation is a foundational task in computer vision, focusing on translating input images from a source domain to a target domain while preserving core semantic content \citep{saharia2022palette, pang2021imagetoimagetranslationmethodsapplications}. The importance of this paradigm is evidenced by its wide-ranging applications, which span critical tasks such as image restoration \citep{zheng2024diffuir, li2024foundir} (e.g. image deraining and image denoising), super-resolution \citep{SR3}, image style translation \citep{choi2021ilvrconditioningmethoddenoising,meng2022sdeditguidedimagesynthesis}, as well as image inpainting \citep{lugmayr2022repaintinpaintingusingdenoising}.  

Early approaches to I2I transformation have been dominated by Generative Adversarial Networks (GAN) \citep{GAN} \citep{gatedgan, cyclegan}. However, GANs suffer from training instability and limited mode coverage \citep{mescheder2018trainingmethodsgansactually}. More recently, denoising diffusion models have set new benchmarks for output quality and diversity by learning a reverse process of iteratively adding and removing noise \citep{NEURIPS2020_DDPM, dhariwal2021diffusion, lipman2022flow}. Early diffusion-based I2I methods, such as SR3 and WeatherDiff \citep{SR3,weatherdiff}, typically initiated  the reverse process from pure Gaussian noise, using the input image solely as a conditioning signal to guide the generation. To more stably preserve structural information of the input and reduce inference uncertainty, advanced approaches \citep{liu2024rddm,luo2023IRSDE,I2SB,indi} no longer initialize from pure noise, instead, they start from noise-carrying input image. This strategy drives the model to \textit{perform denoising and the required domain transformation (e.g., residual removal) simultaneously within a single, coupled reverse process}.


\begin{figure*}[t]
    \centering 
    \includegraphics[width=1\textwidth]{pic/second_page.png}
    \caption{\textit{Motivation of our DDIT.} Here LQ denotes the low-quality image, and HQ denotes the high-quality image. Comparing traditional method \citep{liu2024rddm} with our decoupled approach,  both methods start with multi-task degraded images, followed by the addition of Gaussian noise to obtain LQ+Noise domain. RDDM adapts directly from LR+Noise to the HQ domain, while DDIR first performs residual removal in domain harmonized space, then conducts denoising sampling.}
    \label{fig:intro}
\end{figure*}



However, this coupled sampling from noise-carrying image introduces a critical, yet often overlooked problem: \textbf{the entanglement of domain transformation and noise removal within a single diffusion process.} \green{The coupling process, while being proved effective, can be problematic for unified image transformation task since: (i) Limited unified ability. One of the biggest challenges in unified image transformation is how to perform transformations for multiple distinct distributions in one model, as these distributions often do not overlap and are far apart (See Fig. \ref{fig:intro}-1). Adding noise can effectively reduce the distributional gap across tasks (See Fig. \ref{fig:intro}-2). However, due to coupling reverse process, the model gradually reduces noise intensity, eroding to dealing with difficult distribution transformations.} (ii) Data Inefficiency. Paired degraded-clean images are necessary in traditional training paradigms, but these images are often difficult to obtain \citep{gong2020learningzoominlearningzoomout}. Moreover, artificially synthesized training data often has poor generalization \citep{cai2019realworldsingleimagesuperresolution, liao2024denoising}, leading to inefficiencies in utilizing high-quality training data.


% However, this coupled sampling from noise-carrying image introduces a critical, yet often overlooked problem: \textbf{the entanglement of domain transformation and noise removal within a single diffusion process.} The coupling process, while being proved effective, can be problematic for unified and cross domain image transformation task since: (i) Erosion of domain-gap reduction benefits. The beneficial domain gap reduction effects, achieved through noise injection, will gradually fade as the noise is removed during the reverse process, potentially eroding its benefit before the semantic degraded-to-clean mapping is complete. (ii) Data Inefficiency. Paired degraded-clean images are necessary in traditional training paradigms, but these images are often difficult to obtain \citep{gong2020learningzoominlearningzoomout}. Moreover, artificially synthesized training data often has poor generalization \citep{cai2019realworldsingleimagesuperresolution, liao2024denoising}, leading to inefficiencies in utilizing high-quality training data.
% 尽管这些方法在各自场景中效果显著，基于扩散的图像条件生成却难以在统一参数设置（同一模型与相同采样/引导超参数）下同时胜任多种生成任务。根本原因在于：现有方法通常在同一反演过程中同步完成去噪与残差补偿，将低频语义与高频细节一并处理，易使模型对特定退化形成偏好，从而过拟合于某一类任务。例如，用一套统一配置推理时，模型可能在去抖上表现出色，却在去雨任务上明显欠佳。
% Despite their strong performance in specific tasks, diffusion-based image transformation struggles to handle multiple generation tasks under a unified parameterization (i.e., the same model with identical sampling and guidance hyperparameters). 
% Although these methods address task-specific image restoration well, recent all-in-one restoration models \citep{jiang2024autodir, luo2024daclip, zheng2024diffuir, ai2024multimodalpromptperceiverempower} focus on handling multiple generation tasks within a single model, providing a more practical solution than conventional task-specific approaches without the costly per-degradation retraining. The key challenge is that degradation types have intrinsically conflicting objectives. For instance, low-light enhancement requires brightening an image by amplifying signals, while deraining necessitates removing certain frequency components. To solve this, noteable works employ visual or language-based prompting, contrastive learning, and others.
% Despite their success, We summarize two limitations
% in current approaches. First, existing methods typically couple denoising with residual compensation along the single reverse sampling process, jointly altering low-frequency semantics and high-frequency details, leading to bias toward specific degradations and single-task overfitting. Second, current solutions \citep{potlapalli2023promptir, instructIR,luo2024daclip} often explicitly incorporate degradation information into their models. 
% Such reliance on explicit guidance leads to complex, multi-partite architectures that lack robustness to unseen degradation mixtures, and need many text-image pairs for training. 
% 尽管这些方法在特定任务的图像复原上表现良好， 近期的一体化图像复原任务又提出了新的挑战, which aims to handle different image restoration tasks on a single model. 其关键挑战在于，不同退化类型在目标上天然相互冲突：例如，低照度增强需要通过放大信号来增亮图像，而去雨则需要移除特定频率成分。为了解决这些冲突，一些具有代表性的工作采用了视觉或语言提示（prompting）、对比学习, shared distribution term等策略。 尽管取得了进展，我们归纳出当前一体化图像复原方法的两个局限。其一，现有方法通常在单一的反向采样过程中耦合去噪与残差补偿，从而同时改变低频语义结构与高频细节，这容易导致对特定退化的偏置以及单任务过拟合。其二，现有方案 \citep{potlapalli2023promptir, instructIR, luo2024daclip} 往往显式地将退化信息纳入模型。对这类显式引导的依赖，使得模型架构趋于多组件、复杂化，对未见过的退化混合缺乏鲁棒性，并且训练时需要大量文本—图像配对数据
% Although task-specific image restoration methods perform well, the recent universal image restoration task introduces new challenges, which aims to handle diverse restoration tasks within a single model. The key challenge is that different degradation types have inherently conflicting objectives \citep{tian2025dfpir, ai2024multimodalpromptperceiverempower}. For example, low light enhancement brightens an image by amplifying signals, whereas deraining removes certain frequency components. To mitigate these conflicts, notable works have explored visual or language based prompting, contrastive learning, and shared distribution terms \citep{zheng2024diffuir}. Despite this progress, we identify two limitations of current all-in-one restoration approaches. First, current methods simultaneously alter low-frequency structures and high-frequency details, which tends to bias the model toward particular degradations and leads to single-task overfitting. Second, many solutions \citep{potlapalli2023promptir, instructIR, luo2024daclip} explicitly inject degradation information into the model. Such reliance on explicit guidance results in multi component and complex architectures that are less robust to unseen mixtures of degradations.

%讲一下过去的方法是怎么做image trasnformation的，从噪声出发的方法解决了...的问题，但是带来了新的三个问题（1）（2）erosion of domain-gap reduction benefits，不仅体现在图片domain gap上，也体现在对于残差的gap上（3）数据层面 必须要用成对的数据来训练。 为了解决                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                           




%  RDDM argues that image synthesis can be modeled along two paths: residual diffusion, a directional diffusion from the target image toward the conditional input and noise diffusion focus on generating random details. Meanwhile, recent studies in diffusion models have converged on a coarse-to-fine paradigm: first synthesizing low-frequency structure and then refining high-frequency details \citep{VAR2024,freeT2M2025,dcfdiff2025,DiffBIR2023}.
% This motivates us thinking: can we decouple residual and noise diffusion into two consecutive sub-processes to further realize coarse-to-fine generation?

% To address the above limitations, we revisit the generative process from a model design perspective.

% Current diffusion-based restoration methods start from noisy degraded images and simultaneously remove stochastic noise and degradation residuals (e.g., snow, rain streaks) within a single coupled process. To further investigate the contribution of noise and better utilize noising domain, we propose a novel diffusion-based framework that decouples the restoration objective into two independent and sequential sub-tasks: residual removing and image denoising. 
%这里需要稍微再详细地讲解一下解耦的过程，和以往模型的区别，一两句话
% Requires: \usepackage{amsmath}


% This factorization turns noise into a computational workspace where residual removal is simpler and less conflicting across tasks, while denoising leverages strong priors learned from natural images.


% From the t-SNE plot in Figure \ref{fig: intro}, we observe that after adding noise to degraded images, the distributions of the noisy degraded images in the noise domain become closer, indicating that the high-frequency differences across different degradation tasks are smoothed out and the inter-task distinctions are weakened. In that, noise domain serves as a computational workspace: Removing residuals in noise domain smooths task-specific high frequency artifacts and aligns heterogeneous degradations into a shared, unified representation, thereby reducing inter-task gradient conflicts and simplifying residual removal. 
% o decouple low-frequency semantic transformation and high-frequency detailed generation through a customized two stage diffusion design
To address these issues, we introduce Decoupled Diffusion models for Image-to-Image Transformation (DDIT) that fundamentally unbinds residual diffusion and noise diffusion. DDIT decouples single forward diffusion process into two independent and sequential diffusion processes: a noise diffusion stage that injects Gaussian perturbations to high quality images, followed by a residual diffusion stage that models the deterministic target-to-source process, but now within a space with fixed noise level. The reverse diffusion process, as shown in Fig.~\ref{fig:intro}, is decoupled into residual removal stage (2 $\rightarrow$ 3) followed by a denoising stage  (3 $\rightarrow$ 4), where residual-removal is conducted within noise domain.

% where the domain gap across different transformation tasks and image domain are both reduced.
Our decoupled diffusion approach resolves previous two challenges. First, noise space reduces the gap across various transformation tasks and the difference between degraded and clean images. From Fig. \ref{fig:intro}, we observe that after adding noise, the distances between various types of low-quality images become closer (comparing 1 and 2). In that, noise domain serves as a harmonized computation workspace: Removing residuals in noise domain aligns heterogeneous distributions into a shared, unified representation, thereby reducing inter-task gradient conflicts. Second, it greatly improves data efficiency as the denoising network is trained exclusively on clean images, without the requirement of degraded counterparts. 
Theoretical and empirical results jointly demonstrate that our decouple approach is compatible with multiple popular diffusion paradigms, including DDPM \citep{NEURIPS2020_DDPM}, DDIM \citep{song2022ddim}, and score matching \citep{song2021scorebased}. 
% In that, we can easily plug in powerful pre-trained diffusion models, or train a general denoiser to guide the denoising process.
% Comparing to prior single stage residual denoising approaches \citep{liu2024rddm, luo2023IRSDE, lugmayr2022repaintinpaintingusingdenoising}, the key innovation of our approach lies in designing independent yet sequential updates of residual and noises, thereby improving interpretability and solve existing challenges. 



% 版本1
% From the T-SNE plot in Figure 2, we observe that after070
% adding noise to low quality images, the distributions of the071
% low quality mages in the noise domain become closer, in-072
% dicating that the high frequency differences across distinct073
% degradation tasks are smoothed out and the inter-task dis-074
% tinctions are weakened. In that, noise domain serves as a075
% harmonized computation workspace: Removing residuals076
% in noise domain aligns heterogeneous degradations into a077
% shared, unified representation, thereby reducing inter-task078
% gradient conflicts. In the second stage, the network learns a079
% simple denoising process, rather than a complex task-specific080
% transformation for each degradation. In that, we can easily081
% plug in powerful pre-trained diffusion models, or train a082
% general denoiser to guide the denoising process. To sum083
% up, our decoupled diffusion approach offers two significant084
% advantages: it aligns different task distributions into a shared085
% space, and transfer images back into high quality domain086
% through a simple denoising process.





%!!!!!!!感觉这两段的说理很重复


% 1.下一个结论：噪声是否有用？例如：噪声对无条件的图像生成任务有用，对有条件的图像恢复任务有用。

% 2.噪声为什么有用？机理是什么？解耦之后是否能够讲清楚“噪声有用的机理”？
% 好处：在噪声域中可以进行一个统一的恢复






%那么，好处是什么呢？
% 解耦的好处在all-in-one上的体现，先简单讲一下challenge


% 解耦的好处在少量数据集上的体现
% The decoupled design isolates denoising as a task-free module, independent of any specific degradation. This lets us plug in denoisers pretrained on natural-image corpora at the denoising stage, transferring strong priors and greatly reducing task-specific supervision. Empirically, this yields clear data efficiency: on LOL and All-in-One-3, training with only 25\% of the paired data attains performance within a small margin of the 100\%-data counterparts, indicating that most restoration capacity is inherited from the universal denoiser with only light adaptation.


% 解耦的框架适配于多种任务 inpainting  generation

% Our approach establishes a new benchmark for all-in-one image restoration, enhancing both efficiency and fidelity.
% For the unconditional setting, we simply feed a blank input to the residual-removal stage while keeping the remaining steps unchanged from conditional restoration.
% 解耦的框架适配于不同的生成范式 DDIM DDPM flow-matching SDE
% 移到前面去说？ 一开始就说会更合适






%总结我们的contribution
%1. 提出了一个解耦的框架，更好地解释噪声的作用。通过先在噪声域中去除残差，再去除噪声的造作，在噪声域中进行多任务的融合，不需要每一步加不同scale的噪音去复原，只要在噪声domain去做就会有额外好的效果，实验结果

%2. 该解耦的框架把原来的一个任务分成了两个过程 第二个过程可以被视为从中间段开始的噪声恢复 那么这个过程可以借助传统模型预训练的结果... 实验结果

%3. 我们证实该框架适用于多种不同任务 比如图像inpaiting 生成，并且可以适配现有的不同模型 包括DDPM SDE等


% Image restoration is a critical task with significant applications in diverse domains such as remote sensing, medical imaging, and digital inpainting. The varying degradation patterns encountered in these real-world scenarios demand highly generalizable and robust restoration models. Recently, diffusion models have emerged as a powerful paradigm for image restoration, prized for their strong generative priors.
% Despite this promise, the field meets two obstacles that impede the development of universally applicable restoration systems.

% A fundamental challenge in All-in-One Image Restoration (AiOIR) stems from the conflicting nature of degradation across different tasks. For instance, low-light enhancement requires brightening an image by amplifying signals, while deraining necessitates removing certain frequency components (rain streaks). To mitigate this inherent interference, prevailing solutions often explicitly incorporate degradation information into their models. 
% %这里多讲两句
% However, this reliance on explicit guidance frequently leads to complex, multi-partite architectures that lack robustness to unseen degradation mixtures, which ultimately limits their generalization and practical performance.




% However, current diffusion-based image restoration approaches are predominantly constrained by the limited scale of available training datasets. Besides, these methods typically require sophisticated multi-task processing modules (\cite{zheng2024diffuir}, \cite{luo2024daclip}) to address diverse image degradation patterns, which consequently restricts the model's generalization capability and practical performance in real-world applications.

% Traditional diffusion based iamge degragation approaches(\cite{weatherdiff}) restore images from pure noise, while recent methods like RDDM(\cite{liu2024rddm}) and IR-SDE(\cite{luo2023IRSDE}) start diffusion process from the degraded image. By combining noise diffusion with residual learning, they improved restoration performance. 
% %他们构建了一个更简单合理的建模范式
% However, these methods couple residual correction and noise removal into a single process, which brings two major limitations:
% (1) limited interpretability, because the individual contributions of residual and noise reduction cannot be disentangled or explicitly analyzed;
% (2) lack of flexibility, since the two components cannot be independently tuned or designed. This raises a key research question:


% {\centering
% \textit{Can residual correction and noise removal be decoupled to achieve more interpretable and flexible image restoration?}
% }


% In this work, we propose a novel decoupled diffusion-based restoration framework that splits the “remove-degradation” objective into two complementary sub-tasks: removing image residual and denoising. Specifically, by injecting Gaussian noise into degraded images, our framework reduces the complexity of residual correction and enables easy sharing of residual-removal knowledge across tasks, while treating the denoising process as a universal sub-module independent of specific degradation types. This selective decoupling strategy elegantly aligns different task distributions into a shared space and then guides them back into high-quality, task-specific outputs. 







%
  % 右图 38% 宽
  % \begin{subfigure}[t]{0.26\linewidth}
  %   \centering
  %   \includegraphics[width=\linewidth]{figs/right.pdf}
  %   \caption{test2}
  %   \label{fig:right}
  % \end{subfigure}

  % \caption{test3}



\noindent Our principle contributions are listed as follows: 

\begin{itemize}
    % \item We propose a novel decoupled residual diffusion framework. Our decoupled residual diffusion consists of two independent yet sequential transformations: first mapping the target image into the noise domain, and then transporting this noised target to the conditional input within the same noise domain.
    \item We propose DDIT, a novel diffusion framework for image-to-image transformation that decouples the single forward diffusion process into two sequential and independent stages. Such decoupling strategy is compatible with multiple diffusion paradigms and various image transformation tasks.
    \item DDIT minimizes distribution gaps across various transformation tasks and image domains, as well as the distance between input and target images, achieving state-of-the-art performance in several All-in-One benchmarks.
    \item DDIT significantly enhances data efficiency by supporting training on small amount of paired data, as the denoising network is trained solely on clean images with no need of corresponding degraded images.
    % \item We determined the optimal noise level via both theoretical analysis and empirical validation.
    % \item DDIT minimizes distribution gaps across different transformation tasks, image domains as well as distance between input and target images, achieving state-of-the-art performance in several All-in-One benchmarks.
\end{itemize}


% 这里的方法命名感觉有点不好
% In this paper, we introduce a decoupled image restoration framework that separates residual removal and noise into distinct stages rather than handling them simultaneously. We investigate three sequential strategies:
% \textbf{(1) Residual-first (R$\rightarrow$N)}: residual components are removed under noisy conditions before noise elimination.
% \textbf{(2) Alternating (R$\leftrightarrow$N)}: residual and noise is performed interleaved.
% \textbf{(3) Noise-first (N$\rightarrow$R)}: noise is eliminated prior to residual component removal.

% 这里是不是可以简单分析一下哪个更好，或者各自的优势分别在什么地方
% Through extensive experiments, we show that the \textbf{Residual-first (R$\rightarrow$N)} and \textbf{Alternating (R$\leftrightarrow$N)} strategies consistently outperform conventional joint denoising baselines, with R$\rightarrow$N achieving the best performance across multiple datasets. Moreover, the proposed framework attains superior results compared to state-of-the-art methods, not only under unified dataset training but also on diverse tasks such as rain removal, low-light enhancement, and denoising, highlighting its strong capability in multi-task image restoration.


%不同strategy之间的优劣
% Through extensive experiments, we find that the \textbf{Residual-first (R$\rightarrow$N)} and \textbf{Alternating (R$\leftrightarrow$N)} strategies consistently outperform conventional joint denoising baselines across diverse restoration tasks. Residual-first excels at removing embedded artifacts (e.g., rain streaks), which predominantly reside in the high-frequency band. After adding Gaussian noise, these high-frequency residuals are largely attenuated, fostering a shared representation for multi-task learning and thereby simplifying the subsequent residual-removal step. In contrast, the Alternating strategy—iteratively suppressing residuals and noise—performs slightly better on holistic degradations such as haze, likely because Gaussian denoising and holistic restoration share similar priors; alternating updates progressively recover global structure while preserving high-frequency content. Overall, the proposed framework achieves competitive or superior results under a unified training setting and generalizes well to deraining, low-light enhancement, and denoising, underscoring its efficacy for multi-task image restoration.

%在处理多个数据集的时候，我们的模型不需要额外的分类模块（很重要的优势）



%感觉这段写得太长了 需要精简一下









% “不同去退化任务间的知识共享机制”指的是：把去噪、去模糊、去雾、去雨等不同任务，先统一搬到加噪后的“噪声域”里，再在这个共同空间里用同一套网络/参数学习“从噪声中恢复图像”的通用规律，从而实现任务之间的经验互相借用与迁移。

% 为啥能共享？

% 1. 分布被拉近：对退化图像与清晰图像逐步加噪后，高频差异被抹平，二者在噪声域的分布更接近，任务间的差别被“弱化”。

% 2. 学习难度降低：在这个域里，网络主要学“小幅语义校正+去噪”的通用映射，不必为每种退化都学一套复杂的、强任务相关的变换。

% 3. 参数与表征可复用：同样的去残差扩散/反演步骤、同样的低频结构与自然图像先验（边缘、轮廓、纹理统计），可以被不同任务共享；一个任务上的改进（例如更好的结构保持）能帮助其他任务。

% 一句话概括：把不同去退化任务统一到加噪的共同表示空间中，让模型学到任务无关的通用恢复能力，从而实现跨任务的“知识共享”。


%传统做法的一个challenge是 模型很难通过一套参数学会不同的分布该如何转换这件事。
% 所以很多模型会通过prompt/instruction注入的方式去训练模型，在特定的指令下实现不同的分布转换
%而我们模型强调的：”在噪声中去除“很好的规避了这一问题。我们把不同去退化任务统一到加噪的共同表示空间中，让他们学习相似的分布转换。在噪声域中进行残差去除，可以理解成一种比较相似的分布变换。（这里说的是先加入噪声，然后在噪声中去除的好处）

% 而后续的去噪过程本就是不需要关注不同任务的，也可以理解成学习一种统一的分布转换

% 也就是说 我们通过这种解耦的范式，完美地规避了需要对“不同地任务进行不同的分布转换这一工作”

% 为什么RDDM无法知识共享？RDDM同时去除噪声和残差，其实在逐步去除的过程中，又拉大了不同task之间的分布，而diffuir通过强行减去In让不同任务相似，缓解了这个问题，但是并不是很自然的做法








% 我们提出了一个新的结构

% 这个结构可以用在1.

==> sec/2_Related_Works.tex <==
\section{Related Works}




% 总感觉这句话很怪

% \paragraph{Diffusion-Based}


% Recent works {\cite{luo2024daclip},\cite{zheng2024diffuir}} have explored multi-task or unified restoration frameworks that handle diverse degradations within a single model.  DiffUIR maps different degradation distributions to a shared distribution by introducing a flexible Shared Distribution Term (SDT). This approach faces a trade-off between the commonality of degradations and restoration performance, making it difficult to optimize both simultaneously. Upon further analysis, we find that this term is unnecessary in decoupled restoration paradigm. Other approaches {\cite{luo2024daclip} typically rely on an external task classification module. Such designs introduce unnecessary complexity and are not essential for effective image restoration.

%需要说明一个问题：为什么要在图像恢复框架中使用diffusion模型
%在保证还原度的情况下 有更好的生成效果 参考同类论文的写法

%related work的整体结构要怎么设计？
%全文大概框架 
% 1.Abs+Intro 2页多一点点
% 2.related work 加上到3页
% 3.Method 4，5页
% 4.Experiment 6789
% DiffuIR


%第一段
% 单任务图像恢复。 图像恢复旨在从低质量图像中重建出高质量图像。基于Transformer架构的Restormer \citep{Zamir2021Restormer}，通过多头注意力机制与门控单元有效建模图像中的长程依赖关系，提升了复原细节的清晰度。NAFNet \citep{chen2022simple} 通过简化激活函数并构建高效基线，在保持高性能的同时显著降低了计算复杂度。近年来，扩散模型也被应用于该领域：例如WeatherDiff \citep{weatherdiff} 专门针对恶劣天气下的退化恢复；IRSDE \citep{luo2023IRSDE} 将恢复问题转化为随机微分方程中的逆过程求解；而RDDM \citep{liu2024rddm} 通过从噪声与低质图像的混合体中同时去除噪声和残差，实现了更可解释且精细的图像重建。
% \textbf{Single-Task Image Restoration.} Image restoration seeks to recover a high-quality image from its low-quality version. Restormer \citep{Zamir2021Restormer}, based on the Transformer architecture, efficiently models long-range dependencies in images through multi-head attention and gated units, enhancing the clarity of restored details. NAFNet \citep{chen2022simple} simplifies activation functions and establishes an efficient baseline, significantly reducing computational complexity while maintaining high performance. In recent years, diffusion models have also been applied in the field: for instance, WeatherDiff \citep{weatherdiff} specifically targets restoration under adverse weather degradations; IRSDE \citep{luo2023IRSDE} reformulates the restoration problem as solving an inverse process under stochastic differential equations; while RDDM \citep{liu2024rddm}, by removing noise and residuals simultaneously from mixture of noise and low quality image, achieves more interpretable and refined image reconstruction.

% 尽管这些针对特定任务的方法已取得显著性能，但它们对特定退化类型和程度之外缺乏泛化能力。虽然RDDM和IRSDE等模型在多种恢复任务中表现出鲁棒性，但仍需针对不同数据集和任务训练独立的模型副本。为每一种可能的退化类型单独部署模型不仅资源消耗巨大，在实际应用中也往往难以实现。
% Despite the promising performance achieved by these task-specific methods, they lack generalization ability beyond certain types and levels of degradation. Although models such as RDDM and IRSDE demonstrate robust performance across various restoration tasks, they still require training separate model copies for different datasets and tasks. Deploying an individual model for every possible type of degradation is not only resource-intensive, but also often impractical in real-world applications.

\textbf{Image-to-Image Transformation (I2I)} involves learning a mapping from one image domain to another, enabling tasks like image inpainting, style transfer, and restoration. I2I is widely applied in fields like medical imaging restoration, remote sensing, and art creation. Early research efforts primarily focused on GANs \citep{GAN}. Conditional GANs trained for specific tasks have demonstrated outstanding performance in various cross-domain image style translation tasks \citep{zhu2017unpaired, taigman2016unsupervised, liu2019few}. In addition, image inversion techniques and the exploration of editing directions in latent space have further extended the semantic editing capabilities of GANs \citep{andonian2021paint, zhu2020domain}.
Despite their strengths, GANs still struggle with efficiency and convergence stability \citep{mescheder2018trainingmethodsgansactually}, while diffusion models have recently become a popular alternative for image generation and transformation. SR3 \citep{SR3} focuses on super-resolution and pioneers the use of the input image as a condition for sampling from pure noise to a clear image. RePaint \citep{lugmayr2022repaintinpaintingusingdenoising} extends diffusion models to image inpainting using conditional guidance. ILVR and Palette \citep{choi2021ilvrconditioningmethoddenoising, saharia2022palette} unify multiple tasks such as color transfer and cropping at the architectural level, and attempt to perform related processes in the latent space of images. WeatherDiff and \green{DiffBIR} \citep{weatherdiff, DiffBIR2023} apply diffusion models to image restoration. To more effectively maintain the structural information of the input and reduce inference uncertainty, several methods \citep{liu2024rddm,luo2023IRSDE,I2SB,indi} initializes reverse diffusion process from noise-carrying input image instead of pure Gaussian noise, leading to better performance. However, such designs overlookded the entanglement of residual-removal and denoising process, which has difficulty in handling unified multi-task I2I problem and has limitation in data efficiency.

% SR3 leads this line by casting restoration as iterative denoising conditioned via concatenation, where the low quality input is concatenated with the noisy sample to guide refinement toward a high quality image. Moreover, RePaint, and DiffBIR adopt a generative stance that starts from pure Gaussian noise, using conditions to steer sampling and Palette unifies multiple image-to-image tasks. Further, RDDM and IR-SDE relax the pure noise assumption by initializing dynamics from perturbed observations, aligning diffusion trajectories with inverse constraints while retaining stochasticity.
% However, it is challenging for the aforementioned methods to apply the same set of parameters to different restoration tasks, limiting the construction of a unified restoration model. \\
% ; RePaint employs resampling for free-form inpainting; DiffBIR decouples degradation removal and detail synthesis with latent diffusion priors.
% 第二段还有点乱
%All-in-one image restoration(AiOIR) 中最大的挑战是不同的task的修复需要拟合不同的分布转换，他们之间相互干扰。为了解决这个问题，
% \noindent\textbf{All-in-one Image Restoration} 

% \noindent \textbf{All-in-one Image Restoration} aims to solve multiple restoration tasks within a single model. The core challenge is that each task requires different transformations and optimization directions, leading to interference during training.
% Prompt-based methods like PromptIR and InstructIR \citep{potlapalli2023promptir,instructIR} mitigate task interference by using explicit prompts to guide the model for specific degradations. Although effective, these approaches rely on predefined degradation types and manual instructions, limiting their robustness and generalization. Recent methods have sought to overcome this via more adaptive strategies: VLUNet \citep{vlunet} leverages a vision-language model to automatically extract degradation-aware features, enabling flexible restoration without manual input; AdaIR \citep{cui2025adair} introduces adaptive frequency mining and modulation to emphasize task-relevant frequencies; and DFPIR \citep{tian2025dfpir} employs degradation-guided channel shuffling and attention masking to dynamically align features and reduce interference. Despite these advances, existing methods still depend on explicit degradation-aware cues or encoding mechanisms. This continued reliance may hinder generalization compared to an ideal unified model capable of robustly handling unknown or mixed degradations without any explicit prompts.

% 解决数据稀缺问题
% \textbf{All-in-one Image Restoration (AiOIR)} aims to mitigate the mutual interference among different image restoration tasks during training and inference, thereby enabling a single model architecture and parameter set to handle various types of degradation. Meanwhile, It also seeks to improve data efficiency and mitigate the issue of data scarcity by sharing knowledge across image degradation types during training and inference \citep{jiang2025survey}. Early approaches such as PromptIR and InstructIR \citep{potlapalli2023promptir,instructIR} employ explicit prompts to guide the model in addressing specific degradations, which alleviates task interference to some extent but still relies on predefined degradation categories and manual instructions. To further enhance generalization and data efficiency, VLUNet \citep{vlunet} leverages vision-language models to extract degradation-aware features, while AdaIR and DFPIR \citep{cui2025adair, tian2025dfpir} modulate frequency components and rearrange feature channels, respectively. Moreover, DPPD \citep{DPPD} propose a dynamic prompt distribution learning mechanism, achieving more discriminative and input-adaptive restoration.
% Diffusion-based methods have recently emerged as promising solutions for AiOIR, offering strong generative capabilities and high-fidelity restoration across diverse degradation types. \green{Similar to previous approaches, many diffusion-based models \citep{luo2024daclip, jiang2024autodir} guide the restoration process using text or visual prompts that encode specific degradation type information.}  \green{DiffUIR \citep{zheng2024diffuir}，on the other way, reduces specific degradation type dependency via intergrating a shared distribution term, which gradually maps different distribution into a shared one. However, its suppression mechanism may discard useful information, thus limiting restoration performance.}
% In this work, we propose a decoupled diffusion framework that splits the task into two complementary sub-tasks: image residual removal and denoising. 


% \textbf{All-in-one Image Restoration (AiOIR)} tackles mutual interference among tasks to allow simultaneous handling of various degradations, and enhances data efficiency to alleviate data scarcity via cross-task knowledge sharing \citep{jiang2025survey}. Early approaches such as PromptIR and InstructIR \citep{potlapalli2023promptir, instructIR} rely on predefined degradation categories and manual instructions to guide the model, mitigating task interference to some extent. To further enhance generalization and data efficiency, VLUNet, AdaIR, and DFPIR \citep{vlunet, cui2025adair, tian2025dfpir} respectively leverage language-guided features, frequency modulation, and feature rearrangement to capture degradation characteristics. Moreover, DPPD \citep{DPPD} propose a dynamic prompt distribution learning mechanism, achieving more discriminative and input-adaptive restoration. More recently, diffusion-based methods have been dominant paradigm in AiOIR. Among them, DA-CLIP and AutoDIR \citep{luo2024daclip, jiang2024autodir} guide the diffusion and restoration process by encoding degradation information into textual or visual prompts. Moreover, DiffUIR \citep{zheng2024diffuir}, reduces degradation-type dependency by integrating a shared distribution term, however, its suppression mechanism may discard useful information and limit restoration performance. 

% In contrast, we propose a decoupled diffusion framework that splits the task into two complementary sub-tasks: image residual removal and denoising, which proves to be efficient and effective for I2I translation.



% All-in-one image restoration (AiOIR) aims to address multiple image restoration tasks with a single set of parameters, with the biggest challenge being that each task has its own optimal gradient descent direction, which leads to interference during training.

% To address this, prompt learning \citep{potlapalli2023promptir,instructIR} modify the feature space to align with the shared parameter space by incorporating prompts to guide the restoration process. While these approaches improve modularity and task awareness, they often rely on predefined degradation types and rigid priors, leading to reliance on explicit instructions.



% Prompt-based methods—such as PromptIR and InstructIR \citep{potlapalli2023promptir,instructIR}—address task interference by introducing explicit prompts to guide the model for different degradations. While these approaches enhance task awareness, they often depend on predefined degradation types and explicit instructions, which may limit robustness and generalization. To overcome these limitations, recent methods propose more adaptive strategies: VLUNet [VLUNet][REF] utilizes a vision-language model to automatically extract degradation-aware features, enabling flexible restoration without manual type selection; AdaIR [AdaIR][REF] introduces adaptive frequency mining and modulation to highlight task-relevant frequency components for unified restoration; and DFPIR [DFPIR][REF] employs degradation-guided channel shuffling and attention masking to dynamically align feature representations and reduce task interference.

% Although these advances, current methods still rely on degradation-aware cues or explicit encoding, which may limit their generalization compared to a truly unified model that can robustly handle unknown or mixed degradations without any explicit prompts.
%这里先来一段讲prompts的

 % its reliance on these instructions to encode degradation-specific information may limit its robustness compared to a truly unified model that performs well across all degradation types without the need for explicit prompts.
%  VLUNet
%  ADAIR...
% DFPIR...
% Although,,, these approaches require incorporating degradation information into the network to mitigate the interference between different degragation tasks.



% 第三段
% 扩散模型近年来已成为全能图像修复（AiOIR）的重要方法，其在多种退化类型下均展现出强大的生成能力与高保真合成效果。当前常见的设计（如AutoDIR、DACLIP）通常采用全局文本或视觉提示来引导扩散先验，这些提示编码了预设的退化类型。然而，这类方法依赖于全局提示，往往假定退化类型已知且均匀分布，因而缺乏灵活性与泛化能力。为解决该问题，DiffUIR（Zheng et al., 2024）通过一种选择性沙漏映射机制，将强条件引导与共享分布建模相结合，降低了对提示的依赖，但其输入抑制框架丢弃了有用信息，从而限制了修复质量。

% Diffusion models have recently emerged as powerful approaches for AiOIR, offering strong generative capability and high-fidelity synthesis across diverse degradations. 
% A common design \citep{luo2024daclip,jiang2024autodir} is to steer a diffusion prior with global text or visual prompts that encode the presumed degradation type. These methods typically rely on global text or visual prompts, which presuppose known, uniformly distributed degradation types and therefore lack flexibility and generality. To solve this, DiffUIR \citep{zheng2024diffuir} reduces prompt dependence via a selective hourglass mapping that combines strong conditional guidance with shared distribution modeling, yet its input-suppressive framework discard useful information, thus limits restoration quality.

% 在本研究中，我们提出了一种新型解耦式基于扩散的修复框架，将图像退化目标分解为两个互补子任务：去除图像残差与去噪。基于该框架，我们能够在无需显式指令或不同映射策略的情况下实现全能图像修复。
% In this work, we propose a novel decoupled diffusion image transformation framework that splits the task objective into two complementary sub-tasks: removing image residual and denoising. 

% Due to this framework, we can solve all-in-one restoration without explicit instruction or different mapping strategies.



==> sec/3_Method.tex <==
\section{Method}
\label{headings}
\begin{figure*}[t]  % 使用 figure* 环境
    \centering
    \includegraphics[width=0.99\linewidth]{pic/method_image4.png}  % 替换为您的图片路径
    \caption{\textit{Proposed DDIR framework.} DDIR decouples the traditional single forward diffusion process into two sequential and independent process: a noise diffuison stage that inject Gaussian noise into clean image, followed by a residual diffusion stage that conduct deterministic clean-to-degrade transformation, but now within a fixed noise level. The reverse diffusion process is correspondingly decoupled into a residual removal stage and a denoising stage. }
    \label{fig:main_fig}  % 建议添加标签便于引用
\end{figure*}



\subsection{Revisit Residual Diffusion Process}
Recent works \citep{liu2024rddm,luo2023IRSDE,I2SB,indi} have extended the standard diffusion process framework to mixture of residual diffusion and noisy diffusion process, where residual diffusion refers to a deterministic diffusion from the target image to the input image. These approaches treat image transformation as the joint effect of deterministic residual distortion and stochastic noise, and in the forward diffusion process, they add these two components into target images as follows:
\begin{align}
I_t &= I_{t-1} + \alpha_t I_{res} + \beta_t \epsilon_{t-1}, \notag \\
    &= I_{t-2} + (\alpha_{t-1} + \alpha_{t}) I_{res} + (\sqrt{\beta_{t-1}^2 + \beta_t^2}) \epsilon_{t-2}, \notag \\
    &= \dots = I_0 + \bar{\alpha}_t I_{res} + \bar{\beta}_t \epsilon, 
\label{eq:1}
\end{align}


% houjiahe
\noindent where $I_{res}$ denotes the difference between degraded image $I_{in}$ and clean image $I_0$, and $\alpha_t$ and $\beta_{t}$ are coefficients that controlling the residual and noise diffusion, respectively.
Conversely, their reverse processes simultaneously remove residuals and noise from noise-carrying input image, restoring the clean image in a single generative trajectory.


\subsection{Our Method}
% Our method separates the residual removal and noise removal into two completely independent submodules. During the forward diffusion training phase, noise is first added to corrupt the image, followed by the introduction of degradation that further damages the original image. In the reverse diffusion sampling phase, the degradation is first restored in the noise domain, and then the noise is removed.

\paragraph{Decoupled Forward Process.}
DDIT decouples the forward diffision process into two sequential and independent stages: a stochastic \textbf{noise diffusion} followed by a deterministic \textbf{residual diffusion}. Given a paired degraded image $I_{in}$ and clean image $I_0$, the noise diffusion stage perturbs $I_0$ by progressively injecting Gaussian noise as: 
% \vspace{-1mm}
% \begin{align}
% I^{(1)}_{t_1} &= I^{(1)}_{t_1-1} + \beta_{t_1} \varepsilon_{t_1-1}
% = I^{(1)}_{t_1-2} + \sqrt{\beta_{t_1-1}^2+\beta_{t_2}^2}\, \varepsilon_{t_2-2} \notag \\
% &\overset{}{=} I^{(1)}_0 + \sqrt{\sum\nolimits_{i=1}^{t_1}\beta_i^2}\,\varepsilon
% = I^{(1)}_0 + \bar\beta_{t_1}\,\varepsilon, \label{eq:1}
% \end{align}

 %houjiahe 
\vspace{-1mm}
\begin{align}
I^{(1)}_{t} &= I^{(1)}_{t-1} + \beta_{t} \varepsilon_{t-1} \notag \\
&= I^{(1)}_{t-2} + \sqrt{\beta_{t-1}^2+\beta_{t}^2}\, \varepsilon_{t-2} \notag = \cdots\\  
&= I^{(1)}_0 + \sqrt{\sum\nolimits_{i=1}^{t}\beta_i^2}\,\varepsilon
= I^{(1)}_0 + \bar\beta_{t}\,\varepsilon, \label{eq:2}
\end{align}


% \noindent where $\varepsilon_{t_1-1},..., \varepsilon \sim \mathcal N(0,\mathbf I)$, 
% $\beta_{t_1}$ is the noise schecule coefficient
% ($\bar\beta_{t_1}\ = \sqrt{\sum\nolimits_{i=1}^{t_1}\beta_i^2}\ $) and $\beta_{T_1}$ controls the intensity of noise perturbation. $I^{(1)}_{t_1}$ denotes image at the forward diffusion step $t_1$ in the noise diffusion stage. At \(t_1{=}T_1\) (total steps of residual diffusion), the state \(I^{(1)}_{T_1}\) is not pure Gaussian noise but a clean image corrupted by noise.

 %houjiahe 
\noindent where $\varepsilon_{t-1},..., \varepsilon \sim \mathcal N(0,\mathbf I)$, 
$\beta_{t}$ is the noise schecule coefficient
and $\bar\beta_{t}\ = \sqrt{\sum\nolimits_{i=1}^{t}\beta_i^2}$  controls the intensity of noise perturbation. $I^{(1)}_{t}$ denotes image at the forward diffusion step $t$ in the noise diffusion stage. At \(t{=}T\) (total steps of noise diffusion), the state \(I^{(1)}_{T}= I^{(1)}_0 + \bar\beta_{T}\,\varepsilon\) is not pure Gaussian noise but a clean image corrupted by noise.

We then pass this terminal state of diffusion stage to the residual diffusion stage as initial state by setting
\(I^{(2)}_0 := I^{(1)}_{T_1}\) (see Fig.~\ref{fig:main_fig}). 
We define residual as difference between degraded and the clean images: $I_{res} = I_{in} - I_{0}$.
The subsequent stage, residual diffusion, models the deterministic clean-to-degraded process by injecting the residual $I_{res}$: 
% \vspace{-3mm}
% \begin{align}
% I^{(2)}_{t_2} &= I^{(2)}_{t_2-1} + \alpha_{t_2} I_{\text{res}} 
% = \cdots 
% = I^{(2)}_0 + \sum_{i=1}^{t_2} \alpha_i I_{\text{res}} \notag \\
% &= I^{(2)}_0 + \bar\alpha_{t_2} I_{\text{res}} = I^{(1)}_0 + \bar\beta_T + \bar\alpha_{t_2} I_{\text{res}}
% \label{eq:2}
% \end{align}


 %houjiahe 
\vspace{-3mm}
\begin{align}
I^{(2)}_{t} &= I^{(2)}_{t-1} + \alpha_{t} I_{\text{res}} 
= \cdots 
= I^{(2)}_0 + \sum_{i=1}^{t} \alpha_i I_{\text{res}} \notag \\
&= I^{(2)}_0 + \bar\alpha_{t} I_{\text{res}} = I^{(1)}_0 + \bar\beta_t\varepsilon + \bar\alpha_{t} I_{\text{res}}
\label{eq:3}
\end{align}

\noindent where $\alpha_{t}$ is the residual schedule coefficient ( $\bar\alpha_{t}=\sum\nolimits_{i=1}^{t}\alpha_{i}\ $) and $I^{(2)}_{t}$ denotes image at the forward diffusion step t in the residual diffusion stage. When $t=T$ (total steps of noise diffusion) and $\bar\alpha_{T} = 1$, $I^{(2)}_{T}$ yields the final stage, completing the forward process:
\vspace{-2mm}
\begin{align}
I^{(2)}_{T} = I^{(1)}_{T} + I_{\text{res}} 
= I^{(1)}_0 + \bar\beta_T\varepsilon + I_{\text{res}} = I_{in} + \bar\beta_T\varepsilon.
\label{eq:4}
\end{align}

% Due to the decoupling of the reverse generation process, the denoising network specifically focuses on recovering the initial image from noisy conditions. This architecture enables the utilization of well-established pre-trained natural image denoising models to enhance the network's capability for generating missing details. Furthermore, benefiting from such powerful generative prior knowledges, fine-tuning noise diffusion network from these pre-trained natural image denoising models allows our decoupled framework to achieve robust image restoration performance even when trained on limited paired degraded-restored datasets.


\begin{figure*}[t] \centering \begin{minipage}[t]{0.50\textwidth} \begin{algorithm}[H] \setstretch{0.50} \caption{Training Algorithm} \label{alg:algorithm1} \KwIn{Clean image: $I_0$; \\ \quad\quad\quad Degraded image: $I_{in}$; \\ \quad\quad\quad Residual map: $I_{res} = I_{in} - I_{0}$.} \Repeat{\textnormal{converged}}{ $t_1 \sim Uni({T_1}), t_2 \sim Uni({T_2}), \epsilon \sim \mathcal{N}(\bm{0},\bm{I})$; \\ $I_{t_1}^{(1)} = I_0+\overline{\beta}_{t_1}\epsilon$; \\ Min $\mathcal{L}_{\epsilon}(\theta) = \mathbb{E}[\| \epsilon - I_{\epsilon}^{\theta}(I_{t_1}^{(1)}, I_{in}, t_1) \|_1]$; } \Repeat{\textnormal{converged}}{ $I_t^{(2)} = I_T^{(2)}+\overline{\alpha}_{t_2}I_{res}$; \\ Min $\mathcal{L}_{res}(\theta) = \mathbb{E}[\| I_{res} - I_{res}^{\theta}(I_{t_2}^{(2)}, I_{in}, t_2) \|_1]$; } \end{algorithm} \end{minipage} \hfill
\begin{minipage}[t]{0.48\textwidth}
\begin{algorithm}[H]
\setstretch{0.48}
\caption{Sampling Algorithm}
\label{alg:algorithm2}
\KwIn{Degraded image: $I_{in}$. \\}
$\epsilon \sim \mathcal{N}(\bm{0}, \bm{I})$; \\
$I_T^{(2)} = I_{in} + \overline{\beta}_T \epsilon$; \\
\For {$t=T,\dots,1 $}{
    \quad $I_{t-1}^{(2)} = I_{t}^{(2)} - \alpha_t I_{res}^{\theta}(I_{t}^{(2)}, I_{in}, t)$; \\
}
$I_T^{(1)} = I_{0}^{(2)}$; \\
\For {$t=T,\dots,1 $}{
    \quad $    I_{t-1}^{(1)} = I_{t}^{(1)} - (\overline{\beta}_{t} - \overline{\beta}_{t-1}) \mathstrut \cdot I_{\epsilon}^{\theta}(I_{t}^{(1)}, I_{in}, t)$; \\
}

\Return {$I_0^{(1)} \approx I_0 $}
\end{algorithm}
\end{minipage}
\end{figure*}



\noindent\textbf{Decoupled Reverse Process.}
Correspondingly, the reverse process is decoupled into two independent stages: deterministic residual removal and stochastic noise removal. Each stage is managed by a network trained with a distinct objective. 
 
 % In the first stage, We train a residual removal network $ f^{\theta}_{res}(I_{t}^{2},t,I_{in})$. Given current image, timestep and a degraded image, the network learns to predict part of residuals need to be removed in a noisy, task-harmonized space, where each state $I_{t}^{2}$ contains some noise. By performing this ``semantic shift" before any noise is removed, the model mitigates the domain gap across heterogeneous degradation task and different image types.     


 
 %houjiahe 
In the first stage, we aim to remove residuals from $I^{(2)}_{T}$ in Eq.~\ref{eq:3}, which involves estimation of the residuals injected during the forward process.
To this end, we train a residual removal network denoted as $ f^{\theta}_{res}(I_{t}^{2},t,I_{in})$. Given the current image $I_{t}^{2}$, timestep $t$ and the degraded image $I_{in}$, the network learns to predict part of residuals need to be removed in a noisy, task-harmonized space, where each state $I_{t}^{2}$ contains some noise. By performing this ``semantic shift" before any noise is removed, the model mitigates the domain gap across heterogeneous degradation task and different image types.   
 
Using Eq.~\ref{eq:2}, we obtain the estimated target images $I_0^\theta=I_t-\bar{\alpha}_t f_{res}^\theta$. Given $I_0^\theta$ and $f_{res}^\theta$, the generation process of residual removal is defined as:


\vspace{-2mm}
\begin{align}
p_\theta(I_{t-1}^{(2)}\mid I_{t}^{(2)})
&:= q_\sigma(I_{t-1}^{(2)}\mid I_{t}^{(2)}, I_0^\theta, f_{\text{res}}^\theta) \notag \\
&= \mathcal{N}\!\Big(I_{t-1}^{(2)};\, I_0^\theta + \bar{\alpha}_{t-1} f_{\text{res}}^\theta,\, \sigma_{t}^2 \mathbf I\Big),
\label{eq:5}
\end{align}

% \noindent where $\sigma_{t}^2= 0$ since this residual removal process is deterministic.

 %houjiahe 
\noindent where $q_\sigma(I_{t-1}^{(2)}\mid I_{t}^{(2)}, I_0^\theta, f_{\text{res}}^\theta)$ denotes the transfer probability from $I_t^{(2)}$ to $I_{t-1}^{(2)}$. Since this residual removal process is deterministic, we have $\sigma_{t}^2= 0$.
With Eq.~\ref{eq:3} and \ref{eq:5}, $I_{t-1}$ can be sampled from $I_{t}$ via:
\vspace{-2mm}
\begin{align}
    I_{t-1}^{(2)} &= I_{t}^{(2)} - (\bar{\alpha}_{t} - \bar{\alpha}_{t-1}) I_{res}^\theta \notag \\ 
    &\approx I_{t}^{(2)} - \alpha_{t} f_{res}^\theta(I_{t}^{(2)}, I_{in}, t).
    \label{eq:6}
\end{align}


\noindent Next, we train a denoise network $f_{\epsilon}^{\theta}$ which learns to remove stochastic Gaussian noise injected in the noise diffusion process. We derive the reverse process for noise diffusion by approximating the true intractable posterior $p_\theta\big(I^{(1)}_{t-1} \mid I^{(1)}_{t}\big)$ and assume a variational distribution $q$ conditioned on the model's prediction of the noise $\varepsilon^\theta$. Applying Bayes' rule, we factor this distribution as:
\vspace{-2mm}
\begin{align}
\scriptsize 
p_\theta\big(I^{(1)}_{t-1} \mid I^{(1)}_{t}\big)
&\approx q\big(I^{(1)}_{t-1} \mid I^{(1)}_t, \varepsilon^\theta\big) \nonumber \\
&\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!= \mathcal{N} (I_{t-1};\sqrt{\bar{\beta }_{t-1}^2 -\sigma _t^2} \frac{(I_{t}-I_0)}{\bar{\beta }_{t}} ,\sigma _{t}^2\mathbf{I}
 )
\end{align}
\noindent where the mean $\mu_\theta(I^{(1)}_{t}, t)$ is parameterized by the denoising network and variance $\Sigma_\theta(I^{(1)}_{t}, t)$ is 0 according to DDIM. With Eq.~\ref{eq:2} and \ref{eq:7}, the iterative process is:
\vspace{-2mm}
\begin{align}
I_{t-1}^{(1)}
&= I_0 + \sqrt{\bar{\beta}_{t-1}^{2} - \sigma_{t}^{2}}\;\frac{I_{t}^{(1)}-I_0}{\bar{\beta}_{t}} +\sigma_{t}\varepsilon_{t}\ \notag\\
&= (I_{t}^{(1)} - \bar{\beta}_{t} \varepsilon_{t})
   + \varepsilon_{t} \sqrt{\bar{\beta}_{t-1}^{2} - \sigma_{t}^{2}}
   + \sigma_{t} \varepsilon \notag \\
% &= (I_t^{1} - \bar{\beta}_t\varepsilon_t ) + \sqrt{\bar{\beta}_{t-1}^{2} - \sigma_t^{2}}\;\frac{\,(I_t^{1}-(I_t^{1} - \bar{\beta}_t\varepsilon_t ))\,}{\bar{\beta}_t} +\sigma_t\varepsilon_t\   \notag \\
&\approx I_{t}^{(1)} - (\bar{\beta}_{t} - \bar{\beta}_{t-1})\, 
f_{\epsilon}^{\theta}\!\big(I_{t}^{(1)},\, t\big) \quad (\sigma_{t}=0\ )
\end{align}
\noindent The complete sampling algorithm is shown in Alg. \ref{alg:algorithm2}. 
% \begin{align}
% I_{t-1}^{1}
% &= I_0 + \sqrt{\bar{\beta}_{t-1}^{2} - \sigma_t^{2}}\;\frac{I_t^{1}-I_0}{\bar{\beta}_t} \\
% &= \big(I_t^{1} - \bar{\beta}_t \varepsilon\big)
%   + \sqrt{\bar{\beta}_{t-1}^{2} - \sigma_t^{2}}\;\varepsilon
%   \qquad (\text{sub } I_0 = I_t^{1} - \bar{\beta}_t \varepsilon) \\
% &= I_t^{1} - \big(\bar{\beta}_t - \sqrt{\bar{\beta}_{t-1}^{2} - \sigma_t^{2}}\big)\,\varepsilon \\
% &\approx I_t^{1} - \big(\bar{\beta}_t - \sqrt{\bar{\beta}_{t-1}^{2} - \sigma_t^{2}}\big)\,
%   I_{\epsilon}^{\theta}(I_t^{1}, t) \\
% &= I_t^{1} - (\bar{\beta}_t - \bar{\beta}_{t-1})\, I_{\epsilon}^{\theta}(I_t^{1}, t)
%   \qquad (\sigma_t=0\ \text{for DDIM})
% \end{align}


\paragraph{Training Objectives.} We define our training objective of residual-removal stage ${L}_{\text{res}}(\theta)$ as the difference between ${I}_{\text{res}}$ and predicted residual given current step, input image and timestep.
\vspace{-2mm}
\begin{align}
\mathcal{L}_{\text{res}}(\theta) 
&= \mathbb{E}_{t, I_t^{(2)}, I_{\text{res}}} \left[ \left\| I_{\text{res}} -  f_{\text{res}}^\theta(I_t^{(2)},t,I_{in}) \right\|_1 \right].
\end{align}
\noindent The training objective of denoising stage is to minimize the distance between the true noise and the variational approximation one where $\varepsilon \sim \mathcal{N}(0, \mathbf{I})$. This is equivalent to:

\begin{align}
\mathcal{L}_{\epsilon}(\theta) = \mathbb{E}_{t, I^{(1)}_t, \varepsilon} \left[ \left\| \varepsilon - f_{\epsilon}^{\theta}(I_t^{(1)}, t, I_{\text{in}}) \right\|_1 \right].
\end{align}

\noindent The complete training algorithm is shown in Alg. \ref{alg:algorithm1}. 





% \paragraph{Reverse process.}
% Following DDPM, we approximate $p_\theta(I_{t-1}\!\mid I_t)$ with the tractable Gaussian posterior:
% \begin{equation}
% q(I_{t-1}\!\mid I_t, I_0, I_{\mathrm{res}})
% \;=\; \mathcal{N}\!\big(\mu_t,\; \Sigma_t \mathbf{I}\big),
% \label{eq:posterior}
% \end{equation}
% whose mean and variance (via quadratic completion; see Appendix) are
% \begin{equation}
% \Sigma_t \;=\; \frac{\beta_t^2\,\bar{\beta}_{t-1}^2}{\bar{\beta}_t^2},
% \qquad
% \mu_t \;=\; \frac{(I_t-\alpha_t I_{\mathrm{res}})\bar{\beta}_{t-1}^2 + (I_0+\bar{\alpha}_{t-1} I_{\mathrm{res}})\beta_t^2}{\bar{\beta}_t^2}.
% \label{eq:mean-var}
% \end{equation}
% Substituting the forward marginal \eqref{eq:marginal} into \eqref{eq:mean-var} gives an implementation-friendly form:
% \begin{equation}
% \mu_t \;=\; I_t \;-\; \alpha_t I_{\mathrm{res}} \;-\; \frac{\beta_t^2}{\bar{\beta}_t}\,\epsilon,
% \qquad \epsilon\sim\mathcal{N}(0,\mathbf{I}).
% \label{eq:mu-simple}
% \end{equation}

% \paragraph{Model parameterization.}
% We consider two equivalent parameterizations (training details in Appendix):
% \begin{align}
% \text{\(\epsilon\)-prediction:}\quad
% & \epsilon_\theta(I_t,t)\approx \epsilon,\;\; I_{\mathrm{res}}^\theta \text{ predicted by the network}, \nonumber\\[-2pt]
% & \mu_\theta(I_t,t) \;=\; I_t - \alpha_t I_{\mathrm{res}}^\theta - \frac{\beta_t^2}{\bar{\beta}_t}\,\epsilon_\theta(I_t,t),
% \qquad
% \Sigma_t \;=\; \frac{\beta_t^2\,\bar{\beta}_{t-1}^2}{\bar{\beta}_t^2};
% \label{eq:mu-theta}
% \\[4pt]
% \text{Residual-only:}\quad
% & \text{absorb } -\tfrac{\beta_t^2}{\bar{\beta}_t}\epsilon_\theta \text{ into the parameterization of } I_{\mathrm{res}}^\theta.
% \label{eq:res-only}
% \end{align}

% \paragraph{Sampling.}
% We support both stochastic DDPM-style and deterministic DDIM-style updates:
% \begin{align}
% \text{DDPM (stochastic):}\quad
% & I_{t-1} \;=\; \mu_\theta(I_t,t) \;+\; \sqrt{\Sigma_t}\, z,
% \qquad z\sim\mathcal{N}(0,\mathbf{I}),
% \label{eq:ddpm}
% \\[4pt]
% \text{DDIM ($\eta=0$; residual-only):}\quad
% & I_{t-1} \;=\; I_t \;-\; \alpha_t \, I_{\mathrm{res}}^\theta(I_t,t).
% \label{eq:ddim}
% \end{align}

% \paragraph{Training objective (sketch).}
% Match the chosen parameterization with an MSE objective:
% $\|\epsilon-\epsilon_\theta\|_2^2$ for \(\epsilon\)-prediction,
% or $\|I_{\mathrm{res}}-I_{\mathrm{res}}^\theta\|_2^2$ for residual-only,
% using standard noise-level sampling and loss reweighting (Appendix).

% ===================== Appendix (optional in main file) =====================











% The two-stage decoupled reverse generation process enables residual removal sampling to be performed in noisy conditions, where each step of residual diffusion in Equation 3 contains noise, effectively reducing the learning difficulty of degradation semantic transformation for the residual removal network. As illustrated in Figure 10, despite the significant distributional discrepancy between degraded and clear images in their original space, the progressive addition of noise gradually corrupts high-frequency detail information, thereby substantially narrowing their distributional gap. Conducting residual diffusion in noisy conditions facilitates easier degradation semantic transformation, enhancing the structural and contextual semantic consistency of generated images. This noisy-domain degradation semantic transformation can be viewed as a knowledge sharing mechanism across different degradation removal tasks, which we term the Noisy Knowledge Sharing Domain.
% \paragraph{Decoupled Reverse Process}
% In the reverse (inference) stage, we recover a sample from the shared distribution
% initialized as
% \begin{equation}
%   I_T \;=\; I_{\text{in}} \;+\; \bar{\beta}_T \,\epsilon, 
%   \qquad \epsilon \sim \mathcal{N}(0,\mathbf{I}),
%   \label{eq:init}
% \end{equation}
% to the task-specific distribution.

% Following DDPM, we approximate the reverse transition by
% \begin{equation}
%   q(I_{t-1} \mid I_t, I_0, I_{\text{res}})
%   \;=\;
%   q(I_t \mid I_{t-1}, I_0, I_{\text{res}})
%   \frac{q(I_{t-1} \mid I_0, I_{\text{res}})}{q(I_t \mid I_0, I_{\text{res}})} .
%   \label{eq:bayes}
% \end{equation}
% With the forward-process marginals,
% \begin{align}
%   q(I_{t-1}\mid I_0, I_{\text{res}})
%   &= \mathcal{N}\!\big(I_{t-1}; \; I_0 + \bar{\alpha}_{t-1} I_{\text{res}},\; \bar{\beta}_{t-1}^2 \mathbf{I}\big), 
%   \label{eq:prior}\\
%   q(I_t \mid I_{t-1}, I_0, I_{\text{res}})
%   &= q(I_t \mid I_{t-1}, I_{\text{res}})
%    = \mathcal{N}\!\big(I_t;\; I_{t-1} + \alpha_t I_{\text{res}},\; \beta_t^2 \mathbf{I}\big),
%   \label{eq:cond}
% \end{align}
% we obtain (keeping only the exponential term)
% \begin{align}
%   q(I_{t-1}\mid I_t, I_0, I_{\text{res}})
%   &\propto 
%   \exp\!\left(
%   -\frac{1}{2}
%   \Big[
%     \frac{(I_t - I_{t-1} - \alpha_t I_{\text{res}})^2}{\beta_t^2}
%     + \frac{(I_{t-1} - I_0 - \bar{\alpha}_{t-1} I_{\text{res}})^2}{\bar{\beta}_{t-1}^2}
%     - \frac{(I_t - I_0 - \bar{\alpha}_t I_{\text{res}})^2}{\bar{\beta}_t^2}
%   \Big]
%   \right) \nonumber\\
%   &= \exp\!\left(
%   -\frac{1}{2}
%   \Big[
%     \Big(\frac{\bar{\beta}_t^2}{\beta_t^2 \bar{\beta}_{t-1}^2}\Big) I_{t-1}^2
%     - 2
%       \Big(
%         \frac{I_t - \alpha_t I_{\text{res}}}{\beta_t^2}
%         + \frac{\bar{\alpha}_{t-1} I_{\text{res}} + I_0}{\bar{\beta}_{t-1}^2}
%       \Big) I_{t-1}
%     + C(I_t, I_0, I_{\text{res}})
%   \Big]
%   \right),
%   \label{eq:quad}
% \end{align}
% where $C(\cdot)$ does not depend on $I_{t-1}$.

% The quadratic form in \eqref{eq:quad} identifies a Gaussian
% \(
% \mathcal{N}(I_{t-1}; \mu_t(x_t, I_0, I_{\text{res}}), \Sigma_t(x_t, I_0, I_{\text{res}})\mathbf{I})
% \)
% with mean and variance
% \begin{align}
%   \mu_t(x_t, I_0, I_{\text{res}})
%   &= 
%   \left(
%     \frac{I_t - \alpha_t I_{\text{res}}}{\beta_t^2}
%     + \frac{\bar{\alpha}_{t-1} I_{\text{res}} + I_0}{\bar{\beta}_{t-1}^2}
%   \right)
%   \bigg/
%   \left(
%     \frac{\bar{\beta}_t^2}{\beta_t^2 \bar{\beta}_{t-1}^2}
%   \right),
%   \label{eq:mean1}\\
%   \Sigma_t(x_t, I_0, I_{\text{res}})
%   &= \frac{\beta_t^2 \bar{\beta}_{t-1}^2}{\bar{\beta}_t^2}.
%   \label{eq:var}
% \end{align}

% Using the closed form of the forward process,
% \( I_0 = I_t - \bar{\alpha}_t I_{\text{res}} - \bar{\beta}_t \epsilon \),
% \eqref{eq:mean1} simplifies to
% \begin{equation}
%   \mu_t(x_t, I_0, I_{\text{res}})
%   \;=\;
%   I_t \;-\; \alpha_t I_{\text{res}} \;-\; \frac{\beta_t^2}{\bar{\beta}_t}\,\epsilon 
% \;=\; I_t \;-\; \alpha_t \, I_{\text{res}}^\theta 
%   \label{eq:mean2}
% \end{equation}

% \paragraph{Sampling.}
% We start the reverse process from $p_\theta(I_T)=\mathcal{N}(0,\mathbf{I})$ and use
% \(
% p_\theta(I_{t-1}\mid I_t) = q(I_{t-1}\mid I_t, I_0^\theta, I_{\text{res}}^\theta)
% \),
% where \(I_0^\theta = I_t - \bar{\alpha}_t I_{\text{res}}^\theta - \bar{\beta}_t \epsilon_\theta\).

% \textbf{DDPM-style (stochastic):}
% \begin{equation}
%   I_{t-1}
%   \;=\;
%   \mu_t(x_t, I_0^\theta, I_{\text{res}}^\theta)
%   + \sqrt{\Sigma_t(x_t, I_0^\theta, I_{\text{res}}^\theta)}\,\epsilon^{*}
%   \;=\;
%   I_t - \alpha_t I_{\text{res}}^\theta
%   - \frac{\beta_t^2}{\bar{\beta}_t}\,\epsilon_\theta
%   + \frac{\beta_t \bar{\beta}_{t-1}}{\bar{\beta}_t}\,\epsilon^{*},
%   \quad \epsilon^{*}\sim\mathcal{N}(0,\mathbf{I}).
%   \label{eq:ddpm}
% \end{equation}

% \textbf{DDIM-style (deterministic, residual-only):}
% \begin{equation}
%   \,I_{t-1} \;=\; I_t \;-\; \alpha_t \, I_{\text{res}}^\theta 
%   \label{eq:ddim}
% \end{equation}
% which removes only the predicted residual at each step and does not perform explicit noise removal.


















% where the initial state is $z_0^1 = z_0$, $\bar{\beta}_t$ is the time schedule of noise diffusion coefficients, and $z_t^1$ is the state at step $t$ in the noise diffusion process. When $t = T$, the final state $z_T^1$ of the first-stage noise diffusion is the noisy version of the clean image.

% The second stage is \textbf{residual diffusion}, which represents the deterministic bias from the degraded image to the clean image. Specifically, the residual $z_{res}$ is added to the initial state $z_0^2$ of the second stage,


% where the initial state of the second stage $z_0^2$ is the final state of the first stage $z_T^1$, i.e., $z_0^2 = z_T^1$. $\bar{\alpha}_t$ is the time schedule of the residual diffusion coefficients, and $z_{res}$ is the residual between the degraded image $z_{in}$ and the clean image $z_0$,
% \begin{equation}
%     z_{res} = z_{in} - z_0
% \end{equation}
% When $t = T$, with $\bar{\alpha}_T = 1$, the final state $z_T^2$ of the second-stage residual diffusion becomes the degraded image with added noise,
% \begin{equation}
%     z_T^2 = z_0^2 + z_{res} = z_{in} + \bar{\beta}_T \epsilon
% \end{equation}
% This is consistent with prior works where the residual denoising diffusion model maps from the initial state (clean image $z_0$) to the final state (noisy degraded image $z_{in} + \bar{\beta}_T \epsilon$). However, compared with the single-stage forward process $(z_t = z_0 + \bar{\alpha}_t z_{res} + \bar{\beta}_t \epsilon)$ used in prior works, our approach adopts a two-stage forward process decomposition, which better explains the roles of noise and residual in the diffusion model (residual represents the deterministic bias between degraded and clean images, while noise represents the stochastic perturbation in the diffusion process). This also enables the design of a novel reverse generation process that achieves the separation of residual learning and denoising.




\subsection{Variants of Denoising Stage}
In addition to previously introduced decoupled diffusion framework, where both residual-removal and denoising network are training from scratch, we develop three various designs for the denoising stage: 
\begin{description}[leftmargin=*, labelsep=0.5em, itemsep=0.25em, parsep=0pt]
  \item[\textbf{Pretrained priors.}] We initialize the denoising network with weights pretrained on large scale natural image dataset ImageNet.
  \item[\textbf{Frozen denoiser.}] We reuse a denoiser pretrained on a source task and perform zero-shot inference on the target task with all parameters frozen.
  \item[\textbf{Analytical correction.}] We do not rely the denoising module, instead, during the denoising stage we naively subtract the noise that was added in the first step.
\end{description}




==> sec/4_Experiments.tex <==
\section{Experiments}
\label{others}



In the experiment section, we first validate that our decoupled model excels in unified multi-task restoration on the public benchmarks All-in-One5 and CDD11. We also test DDIT's ability to handle multi-type noise restoration across various domains. We then demonstrate the data efficiency of our model using small training datasets. Finally, we show that our model can be effectively adapted to the SDE framework and many different image transformation tasks.

% Then, we evaluated the performance of our model in simultaneously handling super-resolution, completion, and denoising tasks

% Ablation studies

% Parameters and Inference Time

\subsection{Experiment Settings}


\input{table/datasets}



\input{table/All_in_One_5}
% \input{table/CDD_11}

% \input{table/noise_scale}

\textbf{Datasets.} We use a diverse set of widely-used datasets across various I2I transformation tasks. For unified image restoration, we train on AIO-3, AIO-5 and CDD-11 following the popular settings in previous AiOIR papers \citep{DiffBIR2023, tian2025dfpir, vlunet, cui2025adair, luo2024daclip}, which includes various restoration tasks, like deraining, dehazing, debluring, low light enhancement and their combinations. We also contribute a new Multi-Noise and Multi-Domain (MNMD) dataset, which contains various types of noise and covers multiple domains. Additional studies on inpainting (CelebA-HQ \citep{celebahq} ), super-resolution (FFHQ \citep{ffhq} ), and style translation (edges-to-shoes \citep{isola2017image} ) further demonstrate our framework's versatility. Detailed dataset settings can be found in Tab.~\ref{tab:benchmark} and Appendix~\ref{app:more_datasets}.


\noindent\textbf{Metrics.} To fully assess restoration performance, we utilize a range of image quality metrics including both distortion-based fidelity and perceptual quality. 
 Distortion metrics measure pixel-level differences, with PSNR focusing on signal-to-noise ratio and SSIM on structural similarity \citep{ssim}. Perceptual metrics, such as LPIPS \citep{lpips} and FID \citep{fid}, capture the perceptual quality of images by comparing feature space similarities, better reflecting human visual perception.
Following common practices in All-in-One image restoration, all metrics are calculated on RGB channels of the full-resolution images. 

\input{pic/CDD11}

\noindent\textbf{Experiment Settings.} All experiments are implemented on NVIDIA A6000 48GB GPUs.  The network optimization is achieved through an L1 loss function. For data augmentation, we apply random horizontal and vertical flips to all tasks, and additionally perform histogram equalization on low-light images. Unless otherwise specified, the batch size is set to 8, the initial learning rate is 8e-5, and the total number of training steps is 300{,}000. During training, we randomly crop 256×256 patches from the original images after augmentation, which are then used as inputs to the network.
%设备 超参数 参数量   Batch size, learning rate, and training steps depend on the specific tasks and dataset.




% \input{pic/light}
\vspace{-0.5em}
\input{pic/blur}


\subsection{All-in-One Image Restoration}
\input{pic/data_prune_1}



\input{table/MDMT.tex}
% All-in-One-5. 为验证我们方法在处理多种退化类型上的有效性，我们在五任务联合训练设置下进行系统实验，涵盖去模糊、去雾、去雨、去噪声和低光增强任务。与DFPIR和VLUNet的最新研究一致，我们使用同样的数据集训练了一个综合的DDIR模型，并针对这五个不同的恢复任务进行了测试。如表3所示，在保证参数量和推理时间相似的情况下，我们与最新的领先方法DFPIR \citep{tian2025dfpir}相比，我们的DDIR在五个恢复任务上平均的lpips表现提升了百分之7\%。在低光照和去抖动上的视觉结果可见图xx，参数量和推理时间统计详见附录。 
% 值得一提的是，我们基于扩散模型的恢复方法不仅在感知指标上显著超越了以往的方法，而且在逐像素对比指标上也超出了传统模型。


\textbf{All-in-One-5.} To validate the effectiveness of our method in handling various degradation types, we conducted a systematic experiment using a five-task joint training setup, covering deblurring, dehazing, deraining, denoising, and low-light enhancement tasks. Consistent with recent research by DFPIR and VLUNet, we trained a comprehensive DDIR model using the same dataset and tested it on these five restoration tasks. 
Importantly, we further allocate the batch size of 8 to different tasks according to the following strategy for training: 2 samples for dehazing, 1 for low-light enhancement, 1 for deraining, 2 for denoising, and 2 for deblurring. To have better result, we also employ a two-stage training strategy: In the first stage, we train for 150,000 steps with a learning rate of 8e-5 for both the noise and restoration networks. In the second stage, we train for another 150,000 steps with a learning rate of 1e-5.
As shown in Tab. \ref{tab:AllinOne5}, our DDIT outperforms the recent leading method DFPIR \citep{tian2025dfpir} by a 7\% improvement in average LPIPS score across the five tasks under similar parameter size and inference time conditions. The visual results for low-light and debluring tasks can be seen in Fig.~\ref{fig:main_result}, with detailed parameter size and inference time statistics provided in the appendix.
It is worth noting that our diffusion-based restoration method not only significantly outperforms previous methods in terms of perceptual metrics but also surpasses traditional models in pixel-wise comparison metrics. 
\paragraph{CDD-11.}To further evaluate the robustness and generalization of our approach under complex degradation scenarios, we conduct experiments on the CDD-11 \citep{onerestore} dataset, which comprises 11 diverse degradation types-including haze, rain, snow, low-light, and their various combinations. We compare our method with five recent approaches \citep{potlapalli2023promptir, airnet, wgwsnet, onerestore, MOCEIRS} under a unified experimental setup. As illustrated in Fig.~\ref{fig:CDD11}, our DDIT method achieves competitive or superior performance compared to recent SOTA models across most degradation categories. In particular, DDIT demonstrates clear advantages in challenging composite scenarios (e.g., L+H+S, L+H+R), highlighting its strong capacity for handling mixed degradations. 
% In order to more effectively simulate real-world composite image restoration needs, we utilize a unified setup based on the CDD11 dataset, which contains 11 degradation types, including haze, rain, snow, low-light, and their various combinations. The quantitative results and comparison with other methods \ref{} are shown in Fig. \ref{fig:CDD11}.


% 25-11-13
% \paragraph{All-in-One-5.} To validate the effectiveness of our method in handling various image degradation types, we conducted a systematic experiment using a five-task joint training setup (covering deblurring, dehazing, deraining, denoising, and low-light enhancement) on the same dataset as recent studies \citep{tian2025dfpir, vlunet}. To further improve performance, we use specific data allocation and two-stage training (provided in the Appendix). As shown in Tab.~\ref{tab:AllinOne5}, DDIT achieves SOTA performance on most image restoration tasks as well as average results across all tasks. Notably, DDIT consistently outperforms both recent diffusion-based approaches (DA-CLIP \citep{luo2024daclip}, DiffuIR \citep{dcfdiff2025}) and other non-diffusion based (DFPIR \citep{tian2025dfpir}, VLUNet \citep{vlunet}, and AdAIR \citep{cui2025adair}) in all three metrics. In particular, DDIT achieves a significant improvement in perceptual quality, with a 10\% lower (better) LPIPS average compared to the second-best method. This advantage is also clearly reflected in Fig.~\ref{fig:main_result}-a and Fig.~\ref{fig:main_result}-b, where visual results for low-light enhancement and deblurring are presented. In these representative examples, DDIT produces restorations with richer details and fewer artifacts compared to other methods. These results demonstrate the superiority of DDIT framework on unified image restoration benchmarks, highlighting its ability to adapt to various tasks while ensuring stable and high-quality outputs.


% As shown in Tab.\ref{tab:AllinOne5}, our DDIT achieves the best overall performance across five image restoration tasks, with a significant improvement in average LPIPS (0.073) compared to the recent state-of-the-art method DFPIR\citep{tian2025dfpir} (0.081), under similar parameter size and inference time constraints. Notably, DDIT not only excels in perceptual metrics such as LPIPS and FID, but also consistently delivers strong results in pixel-level metrics like SSIM. Visual comparisons for low-light enhancement and deblurring are provided in Fig.~\ref{fig:main_result}, and detailed statistics on model size and inference speed are included in the appendix. These results demonstrate the superiority and generalizability of our unified diffusion-based approach.


% \paragraph{CDD-11.} To further evaluate the robustness and generalization of our approach under complex degradation scenarios, we conduct experiments on the CDD-11 \citep{onerestore} dataset, which comprises 11 diverse degradation types (haze, rain, snow, low-light, and their various combinations). To ensure a comprehensive and fair comparison, we evaluate our method against five recent approaches \citep{potlapalli2023promptir, airnet, wgwsnet, onerestore, MOCEIRS} under a unified experimental setup. The experimental results are shown in Fig.~\ref{fig:CDD11}, DDIT achieves competitive performance compared to recent SOTA models across most degradation categories. In particular, DDIT demonstrates clear advantages in challenging composite scenarios (e.g., L+H+S, L+H+R), where other methods such as PromptIR, WGWSNet, and MoCE-IR-S \citep{potlapalli2023promptir, wgwsnet, MOCEIRS} experience notable performance drops. Furthermore, our approach achieves the highest average SSIM score, and the radar chart clearly shows that the DDIT curve consistently covers the largest area, highlighting its comprehensive superiority and robust adaptability to diverse complex degradations.




\subsection{Multi-Type Denoising across Different Domain}
Recent All-in-One models mainly focus on handling different degradation types with a single set of parameters, but they often overlook the performance drop caused by domain shifts. In our experiments, we demonstrate that sampling for residual removal in the noise space not only reduces conflicts between different degradation types but also alleviates the issue of domain shifts.
To evaluate unified image transformation across diverse visual domains, we establish a new cross-domain benchmark by introducing three types of noise (Gaussian, salt-and-pepper, and Poisson) into datasets from natural images (WED+BSD400), remote sensing imagery (UC-Merced \citep{ucmerced} ), and medical images (BrainWeb \citep{brainweb1, brainweb2, brainweb3} ). This benchmark enables a unified and systematic evaluation of model generalization and robustness under diverse noise patterns and domain shifts.
As shown in Tab. \ref{tab:MDMT}, our proposed model outperforms previous all-in-one restoration methods by an average margin of +0.8 dB in PSNR and +1.2\% in SSIM across all domains. The complete benchmark construction pipeline are detailed in the appendix. 



% \subsection{Single Tasks}
% Our model is capable of both conditional and unconditional image generation tasks. The following experiments demonstrate the quantitative performance of our model on several single image generation tasks, including image inpainting, image translation, and image generation.

% \textbf{Image Inpainting.} Inpainting is the task of filling new content to missing regions of an image. We select the CelebAHQ dataset to train and test the Decouple-RDDM on this task.  Here we set the mask to be irregular and square. The
% inpainted regions must harmonize with the rest such that the overall face is semantically reasonable and has a natural appearance. Visual examples of face inpainting are illustrated in Figure 7. As can be seen, the proposed Decouple-RDDM demonstrates a strong generative capability in restoring masked
% areas while it at the same time maintains consistency with the original image.

% \textbf{Image Translation.} Image translation aims to transform input images from a source domain to a target domain while preserving their core structural content. We utilize the AFHQ \citep{afhq} dataset to train and evaluate the decouple RDDM model on this task, configuring the transformation direction for cross-species conversion from dogs to cats. The translated images must achieve precise species feature transfer while retaining original poses and scene layouts, generating realistic feline images. Figure 9 presents visual examples of species transformation, demonstrating that the proposed decouple RDDM successfully accomplishes morphological conversion from dogs to cats while maintaining structural consistency with the input images. The generated cat facial images exhibit remarkable performance in both detailed textures and visual authenticity.


% \subsection{General conditioned Vision Models}
% To further validate the All-in-One capability of our model, we attempted to unify multiple conditioned vision tasks within the same set of parameters, including image restoration, image translation, and image completion. We refer to this as a General-Purpose Conditioned Vision Model.
\subsection{Data Efficiency}
To evaluate the data efficiency of our DDIT framework, we randomly sub-sample the training set to {75\%, 50\% and 25\%} while keeping the validation set fixed. As shown in Fig.~\ref{fig:data_efficiency}, on two representative datasets (Low-Light and All-in-One3), DDIT achieves better performance than existing baselines, especially under limited data conditions. Notably, as the amount of training data decreases, the relative performance drop of DDIT remains substantially smaller compared to other methods, underscoring the data efficiency of our approach. These results demonstrate that DDIT can effectively maintain restoration quality even with severely reduced training data, highlighting its practical superiority in data-constrained cases.


% We evaluate the data efficiency of our decoupled framework by sub‐sampling the training set at {25\%, 50\%, 75\%, 100\%} while keeping the validation set fixed. In all settings, the denoising stage train from an off-the-shelf model pre-trained on natural images, whereas the remaining components are trained on the pruned sampled data from scratch.


\subsection{Other I2I transformation Tasks}
\textbf{Image Inpainting.} To validate the generalization capability of the proposed framework across different tasks, we conducted inpainting experiments under various settings. Specifically, we evaluated the inpainting performance at different resolutions using two mask patterns (free form and square) on the CelebA-HQ \citep{karras2017progressive} dataset. It is worth noting that free form masks more closely reflect the restoration demands of complex occlusions encountered in real-world scenarios, whereas rectangular masks are typically used to simulate cases in which local image information is entirely missing. Furthermore, we conducted experiments at both 64×64 and 256×256 resolutions to further confirm the model’s adaptability to different input scales. 
As shown in Tab.~\ref{tab:4}, our method achieved the best or second-best results across all configurations, demonstrating its superior performance and robustness under diverse task conditions. 

\subsection{Score-based Diffusion.}
To validate the generalization capability of the proposed method across different diffusion regimes, we incorporated the decoupling strategy into a score-based diffusion model built upon IR-SDE~\citep{luo2023IRSDE}. We evaluate the performance across three tasks: deraining, inpainting, and denoising. As shown in Tab.~\ref{tab:5}, the Decoupled model consistently outperforms the original baseline across all tasks. These results demonstrate that the decoupling mechanism generalizes effectively beyond specific diffusion frameworks, contributing to more stable and transferable representations.


% Through experiments in Tab.\ref{tab:4} and \ref{tab:5}, we instantiate the decoupled modeling under stochastic SDE processes as well as deterministic probability-flow/ODE sampling. Beyond universal degradation removal, the same architecture transfers across heterogeneous image tasks—including inpainting, image-to-image translation, and super-resolution. Comprehensive qualitative and quantitative results on restoration and completion confirm the robustness and versatility of our approach.





\input{table/inpaint_and_generation}
\input{table/sde_rain100H}





\subsection{Ablation Studies}
\textbf{Performance across different sampling steps.}
Model efficiency and restoration quality hinge on the sampling steps. We provide the restoration performance of different sampling steps in Tab.~\ref{tab:ablation}.
\input{table/ablation1}
% In decoupled models, the residual removal model is responsible for directional semantic elimination in the noise domain, while the denoising model is tasked with restoring the data back to the noise-free domain and performing refined restoration. The necessity for a dedicated denoising model, rather than simply subtracting the noise added in the first step, arises because during directional semantic transformation, the residual removal model also exerts some influence on the noise. This perspective has been confirmed by our designed ablation studies.


% \subsection{Unseen data}
% To further validate the proposed method’s generalization capability, we evaluated its performance on unseen data across four representative image restoration tasks: low-light enhancement, deraining, denoising, and deblurring. The corresponding evaluation metrics are presented in Table \ref{tab:unseen_data}. Specifically, the low-light enhancement task was conducted using a combined dataset comprising MEF \citep{ma2015perceptual}, NPE \citep{wang2013naturalness}, and DICM \citep{lee2013contrast}; the deraining task employed the Practical \citep{yang2017deep} dataset; the denoising task utilized the SIDD \citep{abdelhamed2018high} dataset; and the deblurring task was assessed using the RealBlur \citep{rim2020real} dataset.













==> sec/5_Analysis.tex <==
\section{Discussion and Analysis}

% In this section, we first study influence of noise injection level to decoupled diffusion-based image transformation, and then give an analysis of decoupled framwork in frequency perspective.




\subsection{Investigation of Noise Injection Level}
% noise intensity的定义
% calculate的定义
Since many approaches start sampling from noise-carrying input, the intensity of jnjecting noise is critical to overall performance. However, previous works have rarely provided a systematic method to determine the optimal noise level. In this work, we attempt to explore this issue from both theoretical and experimental perspectives.


% To quantify the influence of noise intensity, we calculate the element-wise difference between the noise-injected and noise-free versions within the degraded region and the background, and report its mean-squared loss as the noise-induced distance.
% As illustrated in Figure 8, when noise itensity increases, the MSE distance of the degraded region drops, indicating that the injected noise effectively erases degraded information and facilitates subsequent restoration. However, too much noise also leads to information loss in the original content region, which affect the final restoration quality. To balance this trade-off, we calculated the ratio between the noise-induced distance of degraded and content regions and this ratio reaches its minimum within the noise intensity range of 0.8 to 1.3. In this interval, noise not only sufficiently removes degraded information but also preserves the original content well.



\mytips
 \textbf{Takeaway 1}:  
In our decoupled diffusion-based architecture, the overall performance is highly sensitive to the noise-injection level, where there exhibits a single optimal interval.
\end{tcolorbox}

We conducted quantitative comparisons across All-in-One-5 datasets, as shown in Table 8. The models achieve either the best or second-best performance when the noise intensity is set to 1.0, and the range from 0.8 to 1.3 consistently delivers stable and superior results. 

\input{pic/noise_scale}
% \input{pic/psnr_ratio_scale}


We define two distinct MMD distances:
\begin{equation}
    A(\sigma) = \text{Dist}(P_\sigma^c, P_\sigma^d),      B(\sigma) = \text{Dist}(P_\sigma^d, P_d) 
\end{equation}
where $A(\sigma)$ measures the distance between the distributions of the noise-carrying clean data \(P_\sigma^c\) and noise-carrying degrade data \(P_\sigma^d\) under a given noise level \(\sigma\). $B(\sigma)$ measures the distance between the noisy-carrying input data distribution and the input data distribution \(P_d\). As the noise level \( \sigma \) increases, the value of \( A(\sigma) \) gradually decreases, while the value of \( B(\sigma) \) gradually increases. Our goal is to find a point where \( A(\sigma) \) is not too big (larger distance makes the transformation harder), while \( B(\sigma) \) is not too big either (input information will be corrupted severely).
Thus, we obtain the following optimization objective:
\[
J(\sigma; \lambda) = \lambda \, \widetilde{A}(\sigma) + (1 - \lambda) \, \widetilde{B}(\sigma), \quad \lambda \in [0, 1],
\]
where \(\widetilde{A}(\sigma)\) and \(\widetilde{B}(\sigma)\) represent the normalized values of \(A(\sigma)\) and \(B(\sigma)\), respectively. By minimizing this objective function, we obtain the optimal noise level \(\sigma^{\star}_J = \arg\min_{\sigma \in \Sigma} J(\sigma; \lambda)\). The value of \(\lambda\) can be adjusted based on the desired balance between the two metrics, normally we give equal weight to both terms ($\lambda = 0.5$).




% Conversely, significant deviation from this optimal range results in substantial performance degradation, highlighting a fundamental trade-off. An insufficient degree of noise perturbation (e.g., scale ≤ 0.5) proves inadequate for forming a sufficiently discriminative latent space, thereby impairing the model's capacity to learn effective residual mappings. On the other hand, an excessive noise amplitude (e.g., scale ≥ 1.5) corrupts the informational content of the degraded input, effectively masking the underlying image structure and complicating the residual recovery process. This analysis confirms that the noise scale is not merely a peripheral parameter but a pivotal factor governing the denoising dynamics. The optimal balance is achieved when the introduced perturbation is substantive enough to regularize the learning process and guide the restoration, yet sufficiently constrained to prevent the obliteration of the essential features in the degraded input. This finding provides a principled guideline for configuring the noise scale in similar residual-learning frameworks.


\subsection{Frequency Perspective}
\mytips
 \textbf{Takeaway 2}:  At the first stage of the decoupled diffusion process, high-frequency information is disrupted first, while low-frequency information is gradually affected in the second stage. The gaussian noise helps the model focus on low-frequency features, preventing overfitting to high-frequency details of specific degradations.
\end{tcolorbox}

\begin{figure}[H]
    \centering 
    \includegraphics[width=\columnwidth]{pic/test.pdf}
    \caption{Zoom in for best View.}
    \label{fig:overview}
\end{figure}






==> sec/6_Conclusion.tex <==
\section{Conclusion}

In this paper, we present a Decoupled Residual Denoising Diffusion framework, a novel approach designed for unified and data-efficient I2I transformation (DDIT). Our experiments on 3 unified image restoration tasks and other image transformation tasks (like inpainting and super resolution) show that DDIT achieves SOTA performance in unified and task-specific I2I with no more than 4 steps. We have also shown that our method, using pre-trained parameters, achieves the best results with a small dataset. We believe our decoupled framework paves the way for developing more general and data-efficient diffusion-based I2I systems in the future.




% Extensive evaluations on a variety of benchmarks demonstrate that DDIT achieves state-of-the-art results across All-in-One I2I tasks—including deraining, dehazing, denoising, deblurring, and low-light enhancement. enhancing data efficiency and maintaining competitive inference costs. We believe our decoupled paradigm opens new avenues for building more flexible, robust, and efficient diffusion-based I2I systems in the future.


% Departing from prior diffusion-based I2I methods that entangle semantic transformation and noise removal within a single process, our framework explicitly decouples both the forward and reverse processes into two sequential and independent stages: residual removal and denoising. This structural separation allows the model to first align semantic content in a harmonized noise space before performing stochastic denoising, thereby mitigating inter-task interference and improving generalization across diverse degradation types.

==> table/CDD_11.tex <==
% \begin{table*}[h]
% \centering
% \renewcommand{\arraystretch}{1.2}
% \setlength{\tabcolsep}{2pt}
% \begin{adjustbox}{max width=\textwidth}
% \begin{tabular}{l
% cccccccccc
% cccccccccccccccccccccccc}
% \toprule
% \multirow{2}{*}{\textbf{Method}} 
% & \multicolumn{2}{c}{\textbf{L}} 
% & \multicolumn{2}{c}{\textbf{H}} 
% & \multicolumn{2}{c}{\textbf{R}} 
% & \multicolumn{2}{c}{\textbf{S}} 
% & \multicolumn{2}{c}{\textbf{L+H}} 
% & \multicolumn{2}{c}{\textbf{L+R}} 
% & \multicolumn{2}{c}{\textbf{L+S}} 
% & \multicolumn{2}{c}{\textbf{H+R}} 
% & \multicolumn{2}{c}{\textbf{H+S}} 
% & \multicolumn{2}{c}{\textbf{L+H+R}} 
% & \multicolumn{2}{c}{\textbf{L+H+S}} 
% & \multicolumn{2}{c}{\textbf{Avg.}} \\
% & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM 
% & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM 
% & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM 
% & PSNR & SSIM \\
% \midrule
% AirNet    
% & 24.83 & .778 & 24.21 & .951 & 26.55 & .891 & 26.79 & .919 
% & 23.23 & .779 & 23.21 & .768 & 23.06 & .763 & 25.04 & .883 & 25.07 & .884 
% & 22.85 & .751 & 22.61 & .748 & 23.75 & .814 \\

% PromptIR 
% & 26.32 & .805 & 26.10 & .969 & 31.56 & .946 & 31.53 & .960 
% & 24.49 & .789 & 24.33 & .773 & 24.12 & .770 & 27.93 & .939 & 28.02 & .940 
% & 23.87 & .763 & 23.55 & .759 & 25.90 & .850 \\

% WGWSNet 
% & 24.39 & .774 & 27.90 & \textcolor{second}{\textbf{.983}} & 31.35 & .906 & 31.25 & .906 
% & 23.95 & .772 & 23.70 & .764 & 23.54 & .759 & 27.53 & .890 & 27.60 & .891 
% & 23.30 & .748 & 23.07 & .745 & 26.96 & .863 \\

% WeatherDiff
% & 23.58 & .763 & 21.99 & .943 & 24.85 & .885 & 24.80 & .883 
% & 22.36 & .756 & 22.25 & .750 & 22.10 & .745 & 23.82 & .867 & 23.91 & .869 
% & 21.87 & .732 & 21.60 & .730 & 22.49 & .799 \\

% OneRestore 
% & 26.48 & \textcolor{second}{\textbf{.826}} & 32.52 & \textcolor{first}{\textbf{.990}} & \textcolor{first}{\textbf{34.96}} & .964 & 34.31 & .973 
% & 25.79 & \textcolor{first}{\textbf{.822}} & 25.65 & \textcolor{first}{\textbf{.811}} & 25.44 & \textcolor{first}{\textbf{.808}} & 29.81 & .960 & 29.92 & .961 
% & 25.23 & \textcolor{first}{\textbf{.797}} & 24.93 & \textcolor{first}{\textbf{.793}} & 28.47 & .878 \\

% MoCE-IR-S       
% & \textcolor{second}{\textbf{27.26}} & .824 & \textcolor{second}{\textbf{32.66}} & \textcolor{first}{\textbf{.990}} & 34.31 & \textcolor{second}{\textbf{.970}} & \textcolor{second}{\textbf{35.91}} & \textcolor{second}{\textbf{.980}} 
% & \textcolor{second}{\textbf{26.24}} & .817 & \textcolor{second}{\textbf{26.05}} & .804 & \textcolor{second}{\textbf{26.04}} & .802 & \textcolor{second}{\textbf{29.93}} & \textcolor{second}{\textbf{.961}} & \textcolor{second}{\textbf{30.19}} & \textcolor{second}{\textbf{.962}} 
% & \textcolor{second}{\textbf{25.41}} & .789 & \textcolor{second}{\textbf{25.39}} & .787 & \textcolor{second}{\textbf{29.05}} & \textcolor{second}{\textbf{.881}} \\

% Ours                    
% & \textcolor{first}{\textbf{27.45}} & \textcolor{first}{\textbf{.828}} & \textcolor{first}{\textbf{32.87}} & .990 & \textcolor{second}{\textbf{34.60}} & \textcolor{first}{\textbf{.974}} & \textcolor{first}{\textbf{36.10}} & \textcolor{first}{\textbf{.983}} 
% & \textcolor{first}{\textbf{26.50}} & \textcolor{second}{\textbf{.825}} & \textcolor{first}{\textbf{26.40}} & \textcolor{second}{\textbf{.813}} & \textcolor{first}{\textbf{26.10}} & \textcolor{second}{\textbf{.805}} & \textcolor{first}{\textbf{30.10}} & \textcolor{first}{\textbf{.963}} & \textcolor{first}{\textbf{30.50}} & \textcolor{first}{\textbf{.964}} 
% & \textcolor{first}{\textbf{25.80}} & \textcolor{second}{\textbf{.801}} & \textcolor{first}{\textbf{25.50}} & \textcolor{second}{\textbf{.799}} & \textcolor{first}{\textbf{29.35}} & \textcolor{first}{\textbf{.886}} \\





% \bottomrule
% \end{tabular}
% \end{adjustbox}
% \caption{Comparison to state-of-the-art on 11 degradation types and their average. PSNR (dB, ↑) and SSIM (↑) are reported.}
% \label{tab:full_composite}
% \end{table*}



==> table/cost.tex <==
\begin{table}[htbp]
    \vspace{-0.6em}
    \centering
    \renewcommand\arraystretch{1.1}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{c|l|ccc|c|ccc}
        \hline
        \multirow{1}{*}{\makecell{\textbf{Table A1}}} 
        & \textbf{Method} & \textbf{Para (M)} & \textbf{FLOPs (G)} & \textbf{Step} & \textbf{Latency (s)} & \textbf{SSIM$\uparrow$} & \textbf{LPIPS$\downarrow$} & \textbf{FID$\downarrow$} \\
        \hline
        \multirow{2}{*}{\makecell{\textbf{Non-\\Diff.}}} 
        & AdAIR  & 29 & 145 & 1 & 0.24 & \textcolor{blue}{0.909} & 0.089 & 26.1 \\
        & VLUNet  & 123 & 143 & 1 & 0.74 & 0.904 & 0.096 & 27.9 \\
        \hline
        \multirow{6}{*}{\makecell{\textbf{Diff.}}} 
        & DiffUIR & 145 & 284 & 3 & 0.75 & 0.869 & 0.117 & 33.7 \\
        & DA-CLIP & 174 & 380 & 3 & 0.76 & 0.876 & 0.108 & 20.0 \\
        & RDDM - S & 145 & 278 & 4 & 0.92 & 0.878 & 0.105 & 27.8 \\
        & \rowcolor{gray!15} RDDM - L & 145$\times$2 & 278$\times$2 & 4 & 1.84 & 0.897 & 0.098 & 23.6 \\
        & DRDD - S & 7+35 & 32+69 & 2 + 2 & 0.10+0.23 & 0.908 & \textcolor{blue}{0.080} & \textcolor{blue}{19.6} \\
        & \rowcolor{gray!15} \textbf{DRDD - L} & 7+145 & 32+278 & 2 + 2 & 0.10+0.45 & \textcolor{red}{\textbf{0.916}} & \textcolor{red}{\textbf{0.073}} & \textcolor{red}{\textbf{18.3}} \\
        \hline
    \end{tabular}
    }
    \vspace{-0.6em}
    \label{tab:efficiency_comparison}
\end{table}

==> table/datasets.tex <==
% \begin{table}[t]
% \centering
% \begin{minipage}{0.50\textwidth}
% \centering
% \caption{\textit{Details for All-in-One image restoration benchmarks.}}
% \label{tab:benchmark}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{l|ll|ll}
% \toprule[0.1em]
% \textbf{Task} & \textbf{Training Dataset} & \textbf{Size} & \textbf{Testing Dataset} & \textbf{Size} \\
% \midrule[0.05em]

% % \multirow{2}{*}{Deraining} & Rain100L \citep{rain100} & 200 & Rain100L & 100 \\
% %  & Rain100H & 1800 & Rain100H & 100 \\

% % \midrule[0.05em]
% % \multirow{2}{*}{Denoising} & BSD400 \citep{bsd400} & 400 & CBSD68 & 68 \\
% %  & WED & 4744 &  Urban100 & 100\\


% \multirow{3}{*}{All-in-One-3} & WED+BSD400 \citep{bsd400,Ma2017WED} & 5,144 &  CBSD68 \citep{bsd400} & 68\\
%   & RESIDE-OTS \citep{SOTS} & 72,135 & SOTS \citep{SOTS} & 492\\
% & Rain100L \citep{rain100} & 200 & Rain100L & 100 \\

% \midrule[0.05em]
% \multirow{5}{*}{All-in-One-5} & GoPro \citep{gopro} & 2,111 & GoPro & 1,111 \\
% & WED+BSD400 \citep{bsd400,Ma2017WED} & 5,144 &  CBSD68 \citep{bsd400} & 68\\
%    & LoLV1 \citep{lol} & 485 &  LoLV1 & 15\\
%   & RESIDE-OTS \citep{SOTS} & 72,135 & SOTS \citep{SOTS} & 492\\
% & Rain100L \citep{rain100} & 200 & Rain100L & 100 \\

% \midrule[0.05em]
% \multirow{3}{*}{MNMD} & UC-Merced \citep{ucmerced}  & 17,010 & UC-Merced & 630 \\
%   & WED+BSD400 & 46,296 &  CBSD68 & 204\\
%    &  BrainWeb \citep{brainweb1} & 4,689 &  BrainWeb-test & 174\\
% \midrule[0.05em]
% \multirow{1}{*}{CDD-11} & CDD-11 \citep{onerestore}  & 13,013 & CDD-11 & 2,200 \\
% \midrule[0.05em]
% \multirow{2}{*}{Low-Light} 
%   & LoLV1 \citep{lol} & 485 & LoLV1 & 15\\
% & LOL-VE \citep{rain100} & 400 & LOL-VE & 100 \\
% \bottomrule[0.1em]
% \end{tabular}%
% }
% \end{minipage}
% \end{table}



% \usetikzlibrary{mindmap}
% \begin{tikzpicture}[grow=right, level 1/.style={sibling distance=6cm}, level 2/.style={sibling distance=3cm}]
%   \node {4.1 Performance on I2I Translation Tasks}
%     child { node {Multi-task Unified Restoration.}
%       child { node {All-in-One-5} }
%       child { node {All-in-One-3} }
%       child { node {CDD-11} }
%     }
%     child { node {Single Task I2I Translation in Multi-Domain.}
%       child { node {MNMD} }
%     }
%     child { node {node {Single-Task I2I Translation in Single Domain..}
%       child { node {Image Inpainting.} }
%       child { node {Super Resolution.} }
%       child { node {Image Denoising.} }
%     };
% \end{tikzpicture}

\usetikzlibrary{mindmap}
\begin{tikzpicture}[grow=right, level 1/.style={sibling distance=6cm}, level 2/.style={sibling distance=3cm}]
  \node {\textbf{4.1 Performance on I2I Translation Tasks.}}
    child { node {Single-Task I2I Translation in Single Domain.}
      child { node {\textit{Image Inpainting.}} }
      child { node {\textit{Super Resolution.}} }
    }
    child { node {Multi-task Unified Restoration.}
      child { node {\textit{All-in-One- 5}} }
      child { node {\textit{CDD 11}} }
    };
\end{tikzpicture}



% \usetikzlibrary{mindmap}
% \begin{tikzpicture}[grow=right, level 1/.style={sibling distance=6cm}, level 2/.style={sibling distance=3cm}]
%   \node {Experiment A}
%     child { node {Task 1}
%       child { node {Dataset 1} }
%       child { node {Dataset 2} }
%     }
%     child { node {Task 2}
%       child { node {Dataset 3} }
%       child { node {Dataset 4} }
%     };
% \end{tikzpicture}

% \usetikzlibrary{mindmap}
% \begin{tikzpicture}[grow=right, level 1/.style={sibling distance=6cm}, level 2/.style={sibling distance=3cm}]
%   \node {4.1 Performance on I2I Translation Tasks}
%     child { node {Multi-task Unified Restoration.}
%       child { node {All-in-One-5} }
%       child { node {All-in-One-3} }
%       child { node {CDD-11} }
%     }
%     child { node {Single Task I2I Translation in Multi-Domain.}
%       child { node {MNMD} }
%     }
%     child { node {Single-Task I2I Translation in Single Domain.}
%       child { node {Image Inpainting.} }
%       child { node {Super Resolution.} }
%       child { node {Image Denoising.} }
%     };
  % \node {4.3 Performance on Limited Training Data}
  %   child { node {Task 1}
  %     child { node {All-in-One-3} }
  %     child { node {Low-Light} }
  %   };
  % \node {4.4 Extensions to other Diffusion Paradigms}
  %   child { node {Task 1}
  %     child { node {All-in-One-5} }
  %   };
  % \node {4.5 Investigation of Noise Injection Level}
  %   child { node {Task 1}
  %     child { node {All-in-One-5} }
  %   };






==> table/different_strategies.tex <==
\begin{table*}[t]     
    \centering     
    \caption{Comparison of three different sampling and training strategies in five image restoration tasks. Best results are shown in bold.}     
    \vspace{-2mm}     
    \resizebox{\textwidth}{!}{     
    \begin{tabular}{l|ccc|ccc|ccc|ccc|ccc}         
        \toprule[0.15em]         
        \multirow{2}{*}{\textbf{Single Task}} &          
        \multicolumn{3}{c|}{\textbf{Enhancement}} &          
        \multicolumn{3}{c|}{\textbf{Deraining}} &          
        \multicolumn{3}{c|}{\textbf{Desnowing}} &          
        \multicolumn{3}{c|}{\textbf{Denoising}} &         
        \multicolumn{3}{c}{\textbf{Dehazing}} \\          
        \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(l){14-16}         
        & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$\\              
        \midrule[0.1em]         
        De-R-N & \textbf{25.63} & \textbf{0.917} & \textbf{0.110} & 29.16 & \textbf{0.900} & \textbf{0.141} & 26.66 & \textbf{0.889} & \textbf{0.128} & 34.37 & 0.926 & 0.097 & 26.17 & 0.968 & 0.036 \\         
        De-N-R & 20.98 & 0.783 & 0.371 & 22.52 & 0.608 & 0.396 & 21.65 & 0.675 & 0.367 & 22.92 & 0.446 & 0.706 & 25.27 & 0.953 & 0.042  \\         
        De-RN & 23.20 & 0.879 & 0.152 & \textbf{30.97} & 0.878 & 0.161 & \textbf{27.73} & 0.877 & 0.138 & \textbf{35.08} & \textbf{0.930} & \textbf{0.064} & \textbf{27.88} & \textbf{0.975} & \textbf{0.024} \\          
        \bottomrule[0.1em]     
    \end{tabular}     
    }     
    \vspace{-2mm}     
    \label{tab:all} 
\end{table*}

==> table/noise_scale.tex <==
% \begin{table*}[t]
%     \centering
%     \caption{Comparison of different noise scale on five challenging image restoration datasets. Best results are highlighted in \textcolor{red}{\textbf{red}}, while the second-best results are \textcolor{blue}{\textbf{blue}}.}
%     \vspace{-2mm}
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{l|c|c|c|c|c|c}
%         \toprule[0.15em]
%         \multirow{2}{*}{\textbf{Scale}} &
%         \textbf{Dehazing (SOTS)} &
%         \textbf{Denoising (CBSD68)} &
%         \textbf{Deraining (Rain100L)} &
%         \textbf{Low-Light (LOLv1)} &
%         \textbf{Deblurring (GoPro)} &
%         \textbf{Average} \\
%         \cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(l){6-6}\cmidrule(lr){7-7}
%         & 
%         PSNR / SSIM / LPIPS &
%         PSNR / SSIM / LPIPS &
%         PSNR / SSIM / LPIPS &
%         PSNR / SSIM / LPIPS &
%         PSNR / SSIM / LPIPS &
%         PSNR / SSIM / LPIPS \\
%         \midrule[0.1em]

%         2.0 &
%         27.36 / 0.9524 / 0.0209 &
%         30.98 / 0.8812 / 0.1038 &
%         34.18 / 0.9662 / 0.0259 &
%         21.16 / 0.8362 / 0.1266 &
%         26.97 / 0.8266 / 0.1990 &
%         28.13 / 0.8925 / 0.0952 \\
%         \midrule[0.05em]
%         1.5 &
%         27.55 / 0.9561 / 0.0182 &
%         31.08 / 0.8834 / 0.1015 &
%         34.69 / 0.9681 / 0.0242 &
%         21.21 / 0.8404 / 0.1279 &
%         27.10 / 0.8287 / 0.1932 &
%         28.33 / 0.8953 / 0.093 \\
%         \midrule[0.05em]
%         1.4 &
%         27.93 / 0.9594 / 0.0169 &
%         31.08 / 0.8841 / 0.1029 &
%         34.95 / 0.9696 / 0.0226 &
%         21.39 / 0.8447 / 0.1243 &
%         27.08 / 0.8286 / 0.1932 &
%         28.48 / 0.8973 / 0.09198 \\
%         \midrule[0.05em]
%         1.3 &
%         28.00 / 0.9601 / 0.0165 &
%         31.09 / 0.8850 / 0.1007 &
%         35.21 / 0.9706 / 0.0210 &
%         21.12 / 0.8438 / 0.1247 &
%         27.15 / 0.8307 / 0.1909 &
%         28.52 / 0.8980 / 0.0908 \\
%         \midrule[0.05em]
%         1.2 &
%         27.86 / 0.9601 / 0.0166 &
%         31.06 / 0.8848 / 0.1029 &
%         35.14 / 0.9701 / 0.0224 &
%         21.54 / 0.8463 / 0.1246 &
%         27.10 / 0.8292 / 0.1913 &
%         28.54 / 0.8981 / 0.0916 \\
%         \midrule[0.05em]
%         1.1 &
%         28.04 / 0.9609 / 0.0158 &
%         31.14 / 0.8858 / 0.1011 &
%         35.23 / 0.9710 / 0.0221 &
%         20.54 / 0.8417 / 0.1254 &
%         27.00 / 0.8265 / 0.1922 &
%         28.39 / 0.8972 / 0.0913 \\
%         \midrule[0.05em]
% 1.0 &
%         \textbf{28.52} / \textbf{0.9651} / \textbf{0.0148} &
%         \textbf{31.35} / \textbf{0.8899} / \textbf{0.0957} &
%         \textbf{36.76} / \textbf{0.9774} / \textbf{0.0154} &
%         \textbf{20.89} / \textbf{0.8433} / \textbf{0.1236} &
%         \textbf{28.30} / \textbf{0.8605} / \textbf{0.1591} &
%         \textbf{29.16} / \textbf{0.9072} / \textbf{0.0817} \\

%         \midrule[0.05em]
%         0.9 &
%         27.97 / 0.9610 / 0.0161 &
%         31.16 / 0.8860 / 0.1009 &
%         35.63 / 0.9725 / 0.0195 &
%         20.68 / 0.8444 / 0.1263 &
%         26.98 / 0.8248 / 0.1931 &
%         28.48 / 0.8977 / 0.0912 \\
%         \midrule[0.05em]
%         0.8 &
%         28.01 / 0.9604 / 0.0165 &
%         31.14 / 0.8861 / 0.0993 &
%         35.68 / 0.9729 / 0.0195 &
%         20.67 / 0.8426 / 0.1259 &
%         27.05 / 0.8275 / 0.1900 &
%         28.51 / 0.8979 / 0.0902 \\
%         \midrule[0.05em]
%         0.5 &
%         27.80 / 0.9588 / 0.0165 &
%         31.03 / 0.8844 / 0.1006 &
%         35.78 / 0.9742 / 0.0183 &
%         20.12 / 0.8357 / 0.1332 &
%         26.87 / 0.8205 / 0.1935 &
%         28.32 / 0.8947 / 0.0924 \\
%         \midrule[0.05em]
%         0.3 &
%         26.63 / 0.9483 / 0.0206 &
%         30.70 / 0.8785 / 0.1003 &
%         35.76 / 0.9736 / 0.0190 &
%         20.11 / 0.8325 / 0.1378 &
%         26.72 / 0.8130 / 0.1978 &
%         27.98 / 0.8892 / 0.0951 \\
%         \midrule[0.05em]
%         0.1 &
%         20.06 / 0.8761 / 0.0643 &
%         29.65 / 0.8534 / 0.1193 &
%         34.91 / 0.9682 / 0.0238 &
%         19.46 / 0.8079 / 0.1661 &
%         26.43 / 0.7993 / 0.2170 &
%         26.10 / 0.8610 / 0.1181 \\
%         \bottomrule[0.1em]
%     \end{tabular}
%     }
%     \vspace{-2mm}
%     \label{tab:noise_scale}
% \end{table*}






\begin{table*}[t]
    \centering
    \caption{Comparison of different noise scale on five challenging image restoration datasets. Best results are highlighted in \textcolor{red}{\textbf{red}}, while the second-best results are \textcolor{blue}{\textbf{blue}}.}
    \vspace{-2mm}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|c|c|c|c|c|c}
        \toprule[0.15em]
        \multirow{2}{*}{\textbf{Scale}} &
        \textbf{Dehazing (SOTS)} &
        \textbf{Denoising (CBSD68)} &
        \textbf{Deraining (Rain100L)} &
        \textbf{Low-Light (LOLv1)} &
        \textbf{Deblurring (GoPro)} &
        \textbf{Average} \\
        \cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(l){6-6}\cmidrule(lr){7-7}
        & 
        PSNR / SSIM / LPIPS &
        PSNR / SSIM / LPIPS &
        PSNR / SSIM / LPIPS &
        PSNR / SSIM / LPIPS &
        PSNR / SSIM / LPIPS &
        PSNR / SSIM / LPIPS \\
        \midrule[0.1em]

        2.0 &
        27.36 / 95.24 / 2.09 &
        30.98 / 88.12 / 10.38 &
        34.18 / 96.62 / 2.59 &
        21.16 / 83.62 / 12.66 &
        26.97 / 82.66 / 19.90 &
        28.13 / 89.25 / 9.52 \\
        \midrule[0.05em]
        1.5 &
        27.55 / 95.61 / 1.82 &
        31.08 / 88.34 / 10.15 &
        34.69 / 96.81 / 2.42 &
        21.21 / 84.04 / 12.79 &
        27.10 / 82.87 / 19.32 &
        28.33 / 89.53 / 9.30 \\
        \midrule[0.05em]
        1.4 &
        27.93 / 95.94 / 1.69 &
        31.08 / 88.41 / 10.29 &
        34.95 / 96.96 / 2.26 &
        21.39 / 84.47 / 12.43 &
        27.08 / 82.86 / 19.32 &
        28.48 / 89.73 / 9.20 \\
        \midrule[0.05em]
        1.3 &
        28.00 / 96.01 / 1.65 &
        31.09 / 88.50 / 10.07 &
        35.21 / 97.06 / 2.10 &
        21.12 / 84.38 / 12.47 &
        27.15 / 83.07 / 19.09 &
        28.52 / 89.80 / 9.08 \\
        \midrule[0.05em]
        1.2 &
        27.86 / 96.01 / 1.66 &
        31.06 / 88.48 / 10.29 &
        35.14 / 97.01 / 2.24 &
        21.54 / 84.63 / 12.46 &
        27.10 / 82.92 / 19.13 &
        28.54 / 89.81 / 9.16 \\
        \midrule[0.05em]
        1.1 &
        28.04 / 96.09 / 1.58 &
        31.14 / 88.58 / 10.11 &
        35.23 / 97.10 / 2.21 &
        20.54 / 84.17 / 12.54 &
        27.00 / 82.65 / 19.22 &
        28.39 / 89.72 / 9.13 \\
        \midrule[0.05em]
1.0 &
        \textbf{28.52} / \textbf{96.51} / \textbf{1.48} &
        \textbf{31.35} / \textbf{88.99} / \textbf{9.57} &
        \textbf{36.76} / \textbf{97.74} / \textbf{1.54} &
        \textbf{20.89} / \textbf{84.33} / \textbf{12.36} &
        \textbf{28.30} / \textbf{86.05} / \textbf{15.91} &
        \textbf{29.16} / \textbf{90.72} / \textbf{8.17} \\

        \midrule[0.05em]
        0.9 &
        27.97 / 96.10 / 1.61 &
        31.16 / 88.60 / 10.09 &
        35.63 / 97.25 / 1.95 &
        20.68 / 84.44 / 12.63 &
        26.98 / 82.48 / 19.31 &
        28.48 / 89.77 / 9.12 \\
        \midrule[0.05em]
        0.8 &
        28.01 / 96.04 / 1.65 &
        31.14 / 88.61 / 9.93 &
        35.68 / 97.29 / 1.95 &
        20.67 / 84.26 / 12.59 &
        27.05 / 82.75 / 19.00 &
        28.51 / 89.79 / 9.02 \\
        \midrule[0.05em]
        0.5 &
        27.80 / 95.88 / 1.65 &
        31.03 / 88.44 / 10.06 &
        35.78 / 97.42 / 1.83 &
        20.12 / 83.57 / 13.32 &
        26.87 / 82.05 / 19.35 &
        28.32 / 89.47 / 9.24 \\
        \midrule[0.05em]
        0.3 &
        26.63 / 94.83 / 2.06 &
        30.70 / 87.85 / 10.03 &
        35.76 / 97.36 / 1.90 &
        20.11 / 83.25 / 13.78 &
        26.72 / 81.30 / 19.78 &
        27.98 / 88.92 / 9.51 \\
        \midrule[0.05em]
        0.1 &
        20.06 / 87.61 / 6.43 &
        29.65 / 85.34 / 11.93 &
        34.91 / 96.82 / 2.38 &
        19.46 / 80.79 / 16.61 &
        26.43 / 79.93 / 21.70 &
        26.10 / 86.10 / 11.81 \\
        \bottomrule[0.1em]
    \end{tabular}
    }
    \label{tab:noise_scale}
\end{table*}


==> table/parameters.tex <==
% \begin{table}[htbp]
%     \centering
%     \caption{\textit{Computational resource comparisons: Parameters, FLOPs, and Runtime.} FLOPs are measured on the patch size of
% 256 × 256 × 3, while Runtime are measured on Rain100L testing set. The sampling steps of denoising model and residual-removal model are both 2.}
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{c|l|ccc|c|ccc}
%         \hline
%         & \textbf{Method} & \textbf{Para (M)} & \textbf{FLOPs (G)} & \textbf{Step} & \textbf{Latency (s)} & \textbf{SSIM$\uparrow$} & \textbf{LPIPS$\downarrow$} & \textbf{FID$\downarrow$} \\
%         \hline
%         & AdAIR  & 29 & 145 & 1 & 0.24 & \textcolor{blue}{0.909} & 0.089 & 26.1 \\
%         & VLUNet  & 123 & 143 & 1 & 0.74 & 0.904 & 0.096 & 27.9 \\
%         \hline
%         \multirow{6}{*}{\makecell{\textbf{Diff.}}} 
%         & DiffUIR & 145 & 284 & 3 & 0.75 & 0.869 & 0.117 & 33.7 \\
%         & DA-CLIP & 174 & 380 & 3 & 0.76 & 0.876 & 0.108 & 20.0 \\
%         & RDDM - S & 145 & 278 & 4 & 0.92 & 0.878 & 0.105 & 27.8 \\
%         & \rowcolor{gray!15} RDDM - L & 145$\times$2 & 278$\times$2 & 4 & 1.84 & 0.897 & 0.098 & 23.6 \\
%         & DRDD - S & 7+35 & 32+69 & 2 + 2 & 0.10+0.23 & 0.908 & \textcolor{blue}{0.080} & \textcolor{blue}{19.6} \\
%         & \rowcolor{gray!15} \textbf{DRDD - L} & 7+145 & 32+278 & 2 + 2 & 0.10+0.45 & \textcolor{red}{\textbf{0.916}} & \textcolor{red}{\textbf{0.073}} & \textcolor{red}{\textbf{18.3}} \\
%         \hline
%     \end{tabular}
%     \label{tab:parameters}
% \end{table}
